PC-PG: Policy Cover Directed Exploration for Provable Policy Gradient Learning

Direct policy gradient methods for reinforcement learning are a successful approach for a variety of reasons: they are model free, they directly optimize the performance metric of interest, and they allow for richly parameterized policies. Their primary drawback is that, by being local in nature, they fail to adequately explore the environment. In contrast, while model-based approaches and Q-learning directly handle exploration through the use of optimism, their ability to handle model misspecification and function approximation is far less evident. This work introduces the the Policy Cover-Policy Gradient (PC-PG) algorithm, which provably balances the exploration vs. exploitation tradeoff using an ensemble of learned policies (the policy cover). PC-PG enjoys polynomial sample complexity and run time for both tabular MDPs and, more generally, linear MDPs in an infinite dimensional RKHS. Furthermore, PC-PG also has strong guarantees under model misspecification that go beyond the standard worst case $\ell_{\infty}$ assumptions; this includes approximation guarantees for state aggregation under an average case error assumption, along with guarantees under a more general assumption where the approximation error under distribution shift is controlled. We complement the theory with empirical evaluation across a variety of domains in both reward-free and reward-driven settings.

==> aggregation_proof.tex <==
\section{Proof of Theorem~\ref{thm:main_result_rmax_pg}}

We need to understand the error $\E_{(s,a)\sim d} [\ind(s \in \Kcal)(A^\pi(s,a) - \theta^\star\cdot \bar \phi(s,a))]$, where $\pi$ is some policy and $d$ is some distribution. $\bar \phi$ refers to the centered features $\bar \phi(s,a) = \phi(s,a) - \E_{a'\sim \pi}(\cdot\mid s)[\phi(s,a')]$. Here $\theta^\star$ is the minimizer of 
\[
\theta^\star = \argmin_{\|\theta \|\leq W} \E_{\sa\sim \rho} [(Q^\pi(s,a) - \theta\cdot \phi(s,a))^2].
\] 
%
Breaking the expectation up over aggregate states $z$, we see that

\begin{align*}
\E_{\sa\sim \rho} [(Q^\pi(s,a) - \theta\cdot \phi(s,a))^2] &= \sum_{z\in \Zcal} \E_{\sa\sim \rho}\ind(\phi(s,a) = z) [(Q^\pi(s,a) - \theta\cdot \phi(s,a))^2]\\
&\sum_{z\in \Zcal} \E_{\sa\sim \rho}\ind(\phi(s,a) = z) [(Q^\pi(s,a) - \theta_z)^2].
\end{align*}
%
Consequently, we see that the optimal solution here sets $\theta^\star_z = \E_{\sa\sim \rho}\ind(\phi(s,a) = z) Q^\pi(s,a)$ which we further summarize as $\theta^\star_z = Q_\rho^\pi(z)$. Note that we have assumed here that the norm bound is large enough to make this solution feasible, for which $W \geq \sqrt{|\Zcal|}/(1-\gamma)$ suffices. 

Now we see that 

\begin{align*}
&\E_{(s,a)\sim d} [\ind(s \in \Kcal)(A^\pi(s,a) - \theta^\star\cdot \bar \phi(s,a))] \\
&= \E_{(s,a)\sim d} [\ind(s \in \Kcal)(Q^\pi(s,a) - \theta^\star\cdot \phi(s,a))] - \E_{s\sim d, a\sim \pi} [\ind(s \in \Kcal)(Q^\pi(s,a) - \theta^\star\cdot \phi(s,a))].
\end{align*}

Let us simplify the first term, as the second one will follow similarly. We see that 

\begin{align*}
&\E_{(s,a)\sim d} [\ind(s \in \Kcal)(Q^\pi(s,a) - \theta^\star\cdot \phi(s,a))] \\
&= \sum_{z\in \Zcal}\E_{(s,a)\sim d}\ind(\phi(s,a) = z) [\ind(s \in \Kcal)(Q^\pi(s,a) \pm Q^\pi_\rho(z) - \theta^\star\cdot \phi(s,a))] \\
&\leq \sum_{z\in \Zcal} \E_{(s,a)\sim d} \ind(\phi(s,a) = z) |Q^\pi(s,a) - Q^\pi_\rho(z)| + 0\\%\E_{(s,a)\sim d} [\ind(s\in \Kcal) (Q^\pi_\rho(z) - \theta^\star \cdot \phi(s,a))]   \\
&\leq \sum_{z\in \Zcal}\E_{(s,a)\sim d} \ind(\phi(s,a) = z)\, \epsilon_z = \E_{(s,a)\sim d} [\epsilon_{\phi(s,a)}].% + \sqrt{\E_{(s,a)\sim d}[(Q^\pi_\rho(z) - \theta^\star \cdot \phi(s,a))^2]}
\end{align*}
%
Here the first inequality uses the value of $\theta^\star$ while the second follows by that of $\epsilon_z$. Proceeding similarly for the second term gives the overall bound:
\[
    \E_{(s,a)\sim d} [\epsilon_{\phi(s,a)}] + \E_{s\sim d,a\sim \pi} [\epsilon_{\phi(s,a)}]
\]

==> algorithm_old.tex <==
\section{The \alg Algorithm and Main Results}% with Linear Parameterization}
\label{section:alg}

We now present the EPOC algorithm and the theoretical
guarantees for linear MDPs (using the policy class $\Pi_{linear}$),
and for state aggregation.

To motivate the algorithm, first consider the original objective function:
\begin{equation}\label{eq:obj1}
\textrm{Original objective:} \quad \max_{\pi\in\Pi} V^\pi(s_0;r)
\end{equation}
where $r$ is the true cost function. Simply doing policy gradient descent on
this objective function may easily lead to poor stationary points due
to lack of coverage (i.e. lack of exploration). For example, suppose
$\pi^0$ is a random initial policy used for policy gradient descent. If
the visitation measure $d^{\pi^0}$ has poor coverage over the
state space, this could potential lead to $\pi^0$ already being a
stationary point.

In such cases, a more desirable objective function would be of the form:
\begin{equation}\label{eq:obj2}
\textrm{A wide coverage objective:} \quad \max_{\pi\in\Pi} \EE_{s_0,a_0\sim\rho_{\mix}}\left[ Q^\pi(s_0,a_0;r)\right]
\end{equation}
where $\rho_{\mix}$ is some initial state-action distribution which has wider
coverage of state space. As argued
in~\citep{agarwal2019optimality,kakade2002approximately,scherrer2014local,Scherrer:API},
wide coverage $\rho_{\mix}$ are critical to the success of policy
optimization methods. However, in the RL setting, our agent can only
start from $s_0$.

The idea of our iterative algorithm, EPOC, will be to successively improve both the
current policy $\pi$ and the coverage distribution $\rho_{\mix}$. The
algorithm will start with some policy $\pi^0$ (say random), and it will
work in episodes: at episode $n$, we have $n$ previous
policies $\pi^0, \ldots \pi^n$. Each of these policies $\pi^i$ induces
a distribution $d^{\pi^i}:=d^i$ over the state space. In fact, let us
consider the average state-action visitation measure over \emph{all} of
these previous policies:
\[
\rho_{\mix}^n = \frac{1}{n+1}\sum_{i=0}^n d^i
\]
Intuitively, $\rho_{\mix}^n$ is a crude reflection of the coverage the
algorithm has over state-action space at episode $n$ (by simply using
a flat average of the past). EPOC will then
use $\rho_{\mix}^n$ in the previous
objective~\eqref{eq:linear_policies} with one modification: EPOC will
modify the instantaneous reward function $r$ with a bonus $b^n$ in
order to encourage the algorithm to find a policy $\pi^{n+1}$ which
covers a novel part of the state-action space. EPOC's objective at the
$n$-th iteration will be:
\begin{equation}\label{eq:obj3}
\textrm{EPOC's objective:} \quad \max_{\pi\in\Pi} \EE_{s_0,a_0\sim\rho^n_{\mix}}\left[ Q^\pi(s_0,a_0;r+b^n)\right]
\end{equation}
Let $\pi^{n+1}$ be the approximate solution to this that EPOC
finds. The idea is that EPOC will be able to effectively optimize
over the region where $\rho^n$ has coverage. Furthermore, by
construction of the bonus, the algorithm is encouraged to escape the
current region of coverage to discover novel parts of the state-action space. 

The idea of the proof is that either the algorithm makes progress in
finding a wider cover or it will have found a good policy (from the
original start state of interest, $s_0$).  In terms of model agnostic
learning, as we shall see, EPOC is always optimizing an objective
function (in \eqref{eq:obj3}) regardless of wether or not the linear
MDP modelling assumptions hold or not; it is not evident if there an
underlying objective function for methods such as UCB or Q-learning.


\iffalse
\subsection{The \alg Algorithm}
\label{sec:rmax_pg}
\begin{table}[!th]
\begin{tabular}{cc}
\hspace*{-0.2in}
\begin{minipage}{0.55\textwidth}
\begin{algorithm}[H]
\begin{algorithmic}[1]
\STATE \textbf{Require}: iterations $K$, threshold $\beta$, regularizer $\lambda$
\STATE Initialize $\pi^0(a|s)$ to be uniform
\STATE Estimate $\pi^0$'s feature covariance matrix $ \widehat\Sigma^0$
\FOR{episode $n = 0, \dots K-1$}
	\STATE Set $\rho^n_{\mix} = \sum_{i=0}^n d^{\pi^i} / (n+1)$ \label{line:mixture}
	\STATE Estimate the policy cover's feature covariance \label{line:feature_cov}\\
\begin{center}
 $\widehat\Sigma_\mix = \sum_{i=0}^n  \widehat\Sigma^i + \lambda \mathbf{I}$ \label{eq:covariance_est}
\end{center}
	\STATE Define known set $\calK^n$
\begin{align}
\label{eq:estimate_known}
\hspace*{-0.2in}\calK^n \!=\! \big\{\sa\!:\!\phi\sa^{\top}\big(\widehat\Sigma_\mix\big)^{-1} \phi\sa \leq \beta\big\}
\end{align}
and  set the exploration bonus $b^n$ \label{line:bonus}
\[
{b}^n\sa =  \frac{\one\{ \sa\not\in\calK^n \}}{1-\gamma}
\]
\STATE Policy update (\pref{alg:npg}):  \label{line:npg}
%\[
$\pi^{n+1} = \text{NPG}( \rho^n_\mix, b^n)$
%\]
\STATE Estimate $\pi^{n+1}$'s feature covariance matrix $ \widehat\Sigma^{n+1}$
\ENDFOR
\STATE \textbf{Return} $\pi^{K}$
\end{algorithmic}
\caption{\alg with linear actor-critic}
\label{alg:rmaxpg_linear}
\end{algorithm}
\end{minipage}
&
\begin{minipage}{0.45\textwidth}
\begin{algorithm}[H]
\begin{algorithmic}[1]
\STATE \textbf{Require}: cover $ \rho$, bonus $b$;\\
NPG params: iterations $T$,  stepsize $\eta$, sample size $M$
\STATE Initialize $\pi^0(a|s)$ to be uniform.
\FOR{iteration $t = 0, \dots T-1 $}
	\STATE Critic: approximate $Q^{^t}_{b}$: \label{line:learn_critic}
	\begin{align*}
		\hspace*{-0.2in}\theta^t = \argmin_{\|\theta\|\leq W} \sum_{i=1}^M ( \theta\cdot  \phi(s_i,a_i) - \widehat{Q}^{t}(s_i,a_i) )^2,
	\end{align*} where $s_i,a_i\sim \rho$, and $\widehat{Q}^t (s_i,a_i)$'s are unbiased estimates of $Q^{t}_{b}(s_i,a_i)$
	\STATE Policy update via exponential gradient: \label{line:learn_actor}
    \IF{$s\in \Kcal$}
    \STATE
%	\begin{eqnarray*}
		%\hspace{-0.2in}
\mbox{$\pi^{t+1}(a|s) \!\propto\! \pi^t(a|s) \exp\left(\eta \theta^t\cdot \phi\sa\right)$}%,  \forall s \in \calK\end{eqnarray*}
\ELSE
\STATE
%\begin{eqnarray*}
		%\hspace*{-0.2in}
\mbox{$\pi^{t+1}(\cdot|s) \!=\! \text{Uniform}\left(\{a:\sa\not\in\calK\}\right)$}%, \forall s\not\in \calK.
%	\end{eqnarray*}
\ENDIF
	%
	%
	\ENDFOR
\STATE \textbf{Return} $\pi^{T}$
\end{algorithmic}
\caption{NPG$(\rho,b, \Kcal)$}
\label{alg:npg}
\end{algorithm}
\end{minipage}
\end{tabular}
\end{table}
\fi

\subsection{The \alg Algorithm}

\input{main_pseudocode}
At the high-level, our algorithm iteratively constructs a policy cover, and uses policy optimization from the cover's state distribution as the initial distribution. We design a reward bonus to encourage exploration of novel states and actions not adequately covered. For the bonus, we borrow ideas from linear bandits~\citep{dani2008stochastic,abbasi2011improved} to reward $\sa$ pairs whose features $\phi\sa$ have a small projection on the covariance matrix of the policy cover.  The policy optimizer uses Natural Policy Gradient \citep{Kakade01,Bagnell:2003:CPS:1630659.1630805,Peters:2008:NA:1352927.1352986}.%
%
%We prove that it achieves weakly agnostic results under general MDPs with polynomial sample complexity %under a potentially infinite-dimensional feature mapping $\phi$
%(\pref{sec:rmaxpg_analysis}).


%
%
\textbf{Policy cover and reward bonus.}
At each episode $n$, we maintain an estimate of the feature covariance matrix of $\pi^n$, denoted as:
Note that $\widehat\Sigma^n$ is an unbiased estimate of $\Sigma^n:= \EE_{\sa\sim d^n} \phi\sa\phi\sa^{\top}$. To sample a state-action pair from $d^{\pi}_{\rho}$ with $\rho\in\Delta(S)$ being some initial state distribution, we can sample an $h \in\mathbb{N}$ with probability proportional to $\gamma^h$, and then execute $\pi$ to step $h$ starting from the initial distribution $\rho$.

At the beginning of each episode, we form a \emph{policy cover} $\rho_{\mix}^n$ by averaging all previous policies' distributions and form an estimated covariance matrix  $\widehat{\Sigma}_{\mix}$ (\pref{line:feature_cov}). Next we use this covariance matrix and the linear MDP structure to identify state, action pairs which are adequately covered by $\rho$. Since the $Q$-functions of all policies are linear, if we visit features like $\phi(s,a)$ often under $\rho_{\mix}$, then we can estimate $Q$ values of any policy in $\sa$ easily, say by rollouts. Hence, the goal of the reward bonus is to identify state, action pairs whose features are less explored by $\rho_{\mix}$ and incentivize visiting them. The definition of bonus $b^n(s,a)$ at iteration $n$ of the algorithm shown below achieves this:

\begin{equation}
b^n(s,a) = \frac{\one\{\sa~:~ \phi\sa^\top (\widehat{\Sigma}_{\mix})^{-1}\phi\sa \geq \beta\}}{1-\gamma}.
\label{eq:bonus}
\end{equation}
%
If the quadratic form defining the bonus is large, then $\Sigma_{\mix}$ has a small eigenvalue along $\phi\sa$ and we assign the largest possible future reward from this $\sa$ pair to encourage exploration.\footnote{For infinite dimensional RKHS, Eq.~\ref{eq:bonus} can be computed in the dual using the kernel trick (e.g., \cite{valko2013finite}).} We note that the use of the largest reward in an underexplored state is reminiscent of the Rmax algorithm~\cite{brafman2002r} which does the same in the tabular setting.

The remaining steps of the algorithm perform a slightly modified Natural Policy Gradient (NPG) update to optimize the combined reward $r+b^n$ with $\rho_{\mix}^n$ as the restart distribution. Note we do not need to precompute bonuses for every $\sa$: we just need to compute bonuses along the rollouts generated from the NPG procedure.



\textbf{Policy Optimization.}
We denote $Q^{\pi}_{b^n}$ and $V^{\pi}_{b^n}$ as the $Q$ and value function of policy $\pi$ under reward $r+b^n$. In the $t$-th iteration of the policy optimization inner loop (lines~\ref{line:for_beg}-\ref{line:for_end}), we learn a linear function $\theta^t\cdot \phi\sa$ to approximate $Q^{t}_{b^n}\sa$ (\pref{line:learn_critic}). Specifically, we draw $M$ many samples $(s_i,a_i)\iidsim \rho_{\mix}^n$ and for each $(s_i,a_i)$, we compute an unbiased estimate of $Q^t_{b^n}(s_i,a_i)$. Drawing a state-action pair from $\rho_{\mix}^n$ can be implemented by first uniformly sampling a policy $\pi$ from $\{\pi_0,\pi_1,\dots \pi_n\}$, and then  sampling a state-action pair from $d^{\pi}$. For any $\sa$, to get an unbiased estimate $\widehat{Q}^{\pi}\sa$ of $Q^{\pi}\sa$, we can sample a time step $h\geq 0$ with probability proportional to $\gamma^h$, and roll out our policy $\pi$ from $\sa$ to time step h. We set $\widehat{Q}^{\pi}\sa$ as the undiscounted sum of the rewards along the rollout and then perform constrained linear regression using the $M$ data points to estimate $\theta^t$.

Using $\theta^t$, we update the policy per-state as shown in~\pref{line:learn_actor}. Note that the first equation in ~\pref{line:learn_actor} can be rewritten in an equivalent policy parameter updater step:
\begin{center}
$w^{t+1} := w^{t} + \eta \theta^t$ with $\pi^t\sa \propto \exp(w^t\cdot \phi\sa)$.
\end{center}
%
That is, $\theta^t$ is the natural gradient direction and $\eta$ is the learning rate. For states which have non-zero bonuses, we simply take actions with bonuses uniform randomly (the second equation in \pref{line:learn_actor}).


\textbf{Intuition for tabular setting.}
For a more intuitive understanding of the bonus, let us consider tabular MDPs. In this case, $(\widehat \Sigma_{\mix})^{-1}$ is a diagonal matrix with entries proportional to $1/n_{s,a}$, where $n_{s,a}$ is the number of times  $\sa$ is observed in the data collected to form the matrix $\widehat\Sigma_{\mix}$. Hence the bonus simply rewards state, action pairs with a small number of samples when executing the policy cover, and thereby encourages reaching new states. Policy optimization under NPG for tabular problem decouples across states~\cite{Kakade01,agarwal2019optimality}.

\textbf{On model-free exploration} Typical exploration algorithms for tabular~\cite{kearns2002near,brafman2002r,agrawal2017posterior} as well as linear MDPs~\cite{jin2019provably} implicitly or explicitly build an empirical MDP model and then plan in the model. State, action pairs which are less explored are typically modified to have dynamics leading to a maximally rewarding absorbing state. In contrast \alg plans in the real environment through its policy optimization subroutine. Dynamics of the real world cannot be altered and adding bonus to rewards is the only natural mechanism. This model-free and on-policy nature of our approach, where we do not store all the past data but only incrementally update the policy from its execution in the environment presents technical challenges in the analysis, but also affords robustness to model misspecification as we discuss in the next section.



\subsection{Main Results}
\label{sec:analysis}
For analysis we focus on proving sample complexity results for linear
MDPs with potentially infinite dimensional feature $\phi$. We then
show how our algorithm can work under model misspecification in
arguably one of the most basic models, that of state-aggregation.

\textbf{Well specified case: Linear MDPs.} To measure the sample complexity, we define \emph{intrinsic dimension} of the underlying MDP $\mathcal{M}$.
First, denote the covariance matrix of any policy $\pi$ as $\Sigma^{\pi} = \EE_{\sa\sim d^{\pi}}\left[\phi\sa\phi\sa^{\top}\right]$.%
We define the intrinsic dimension below:
\begin{definition}[Intrinsic Dimension $\widetilde{d}$]
%Intrinsic dimension $\widetilde{d}$:
%\begin{align*}
$\widetilde{d}: =\max_{n\in\mathbb{N}^+} \max_{\{\pi^i\}_{i=1}^n } \frac{  \log\det\left(\sum_{i=1}^n \Sigma^{\pi^i} + \mathbf{I}\right) }{\log(n + 1)}$.
%
%\end{align*}
\label{def:int_dim}
\end{definition}
This quantity is identical the intrinsic dimension in Gaussian
Processes bandits  \citep{srinivas2010gaussian}; one viewpoint of this
quantity is as the information gain from a Bayesian perspective
(\cite{srinivas2010gaussian}). A related quantity occurs in a more
restricted linear MDPs model, in \citet{yang2019reinforcement}. Note
that when $\phi\sa\in \mathbb{R}^d$, we have that
$\log\det\left(\sum_{i=1}^n \Sigma^{\pi^i} + \mathbf{I}\right) \leq d
\log(n + 1)$ (as $\|\phi(s,a)\|_2\leq 1$), which means that the
intrinsic dimension is $d$.  Note that $\widetilde{d}\ll d$ if the
covariance matrices from a sequence of policies only concentrated in a
low-dimensional subspace. 

\begin{theorem}[Sample Complexity of \alg for Linear MDPs]
Fix $\epsilon, \delta \in (0,1)$. Suppose that $\mathcal{M}$ is a linear MDP. %Then $\varepsilon_{bias} = 0$.
There exists a setting of the parameters such that \alg
uses a number of samples at most $\text{poly}\left( \frac{1}{1-\gamma},\log(A), \frac{1}{\epsilon}, \widetilde{d}, W, \ln\left(\frac{1}{\delta}\right) \right)$
and, with probability greater than $1-\delta$, returns a policy $\widehat \pi$ such that:
$V^{\widehat\pi}(s_0) \geq \max_{\pi\in\Pi_{linear}}V^{\pi}(s_0) - \epsilon$. %where $V^{\star}(s_0)$ is the optimal value function.
\label{thm:linear_mdp}
\end{theorem}
The detailed bound with the rates, along with the setup of
hyperparameters $\beta, \lambda$, $T$, $M$, $\eta$ (learning rate in
NPG) are in~\pref{app:rmaxpg_sample}. Our theorem assumes discrete
actions but the sample complexity only scales polylogarithmically with
respect to the number of actions $A$, making the algorithm scalable to
large action spaces. 

\begin{remark}For tabular MDPs, as $\phi$ is a $|\Scal||\Acal|$ indictor vector, the theorem above immediately extends to tabular MDPs with $\widetilde{d}$ being replaced by $|\Scal|\Acal|$ and $\Pi_{linear}$ replaced by $\Pi_{tab}$.
\end{remark}
\begin{remark}
In contrast with LSVI-UCB \citep{jin2019provably}, \alg works for
infinite dimensional $\phi$ with a polynomial dependency on the
intrinsic dimension $\widetilde{d}$. To the best of our knowledge,
this is the first infinite dimensional result for the model proposed
by \citet{jin2019provably}. 
\end{remark}

\begin{remark} \alg can run in reward-free setting in linear MDPs
  (\pref{thm:reward_free} in \pref{app:reward_free_explore}): $r\sa =
  0$, $\forall \sa$. Here, \alg identifies a subset $\Kcal^n$, such
  that the features of every $\sa\in\Kcal^n$ are well explored, while
  no policy can escape $\Kcal^n$ will probability more than
  $\epsilon$. 
\end{remark}


\input{state_aggregation}





==> app_linear_mdp.tex <==
%!TEX root = main.tex

\iffalse
\subsection{Application to Approximate Linear MDPs}
\label{app:app_approx_linear_mdp}

In this section, we prove the agnostic result for mis-specified linear MDPs. Consider a fixed linear MDP $\widehat{M}$ that is defined in \pref{def:linear_mdp}. For any state-action pair $\sa$, let us denote the approximation error $\epsilon_{s,a;\widehat{M}}$ as follows:
\begin{align*}
\max\left\{\left\| P(\cdot | s,a) - \widehat{P}(\cdot | s,a)   \right\|_1,  \left\lvert r\sa - \widehat{\theta}\cdot\phi\sa \right\rvert  \right\} = \epsilon_{s,a;\widehat{M}}.
\end{align*}
Namely we assume that there exists a linear MDP that can approximate the true MDPs up to $\epsilon_{s,a;\widehat{M}}$ for each state-action pair $\sa$.

Given a policy $\pi$, we denote $Q^{\pi}$ as the Q function of $\pi$ under the true MDP and $\widehat{Q}^{\pi}$ as the Q function of $\pi$ under $\widehat{M}$.
The following simulation lemma will be useful. 
\begin{lemma}[Simulation Lemma] For any policy $\pi$, any state-action pair $\sa$,
\end{lemma}
\fi







\subsection{Application to Linear MDPs (Proof of \pref{thm:linear_mdp})}
\label{app:app_to_linear_mdp}

To prove \pref{thm:linear_mdp}, we just need to show that $\varepsilon_{bias}$ defined in \pref{ass:transfer_bias} is zero under the linear MDP model assumption.

For linear MDP $\calM$, we assume the following parameters' norms are bounded:
\begin{align*}
\| v^{\top} \mu  \| \leq \xi \in\mathbb{R}^+, \forall v\in\mathbb{R}^{|\Scal|} s.t., \|v\|_{\infty}\leq 1,  \quad \|\theta\| \leq \omega\in\mathbb{R}^+.
\end{align*}With these bounds on linear MDP's parameters, we can show that for any policy $\pi$, we have $Q^{\pi}\sa = w^{\pi}\cdot \phi\sa$, with $\|w^{\pi}\|\leq \omega + V_{\max} \xi $ \citep{jin2019provably}, where $V_{\max} = \max_{\pi,s}V^{\pi}(s)$ is the maximum possible expected total value ($V_{\max}$ is at most $r_{\max}/(1-\gamma)$ with $r_{\max}$ being the maximum possible immediate reward).

At every episode $n$, recall that NPG is optimizing the MDP $\calM_{b^n} = \{P, r\sa + b^n\sa\}$ with $P, r$ being the true transition and reward of $\calM$ which is linear under $\phi\sa$.

Due to the reward bonus $b^n\sa$ in $\calM_{b^n}$, $\calM_{b^n}$ is not necessarily a linear MDP under $\phi\sa$ ($P$ is still linear under $\phi$ but $r\sa+b^n\sa$ it not linear anymore).
However, augmenting feature vector by one more bit, i.e.,  augment feature vector $\wt{\phi}\sa = [ \phi\sa^{\top}, \one\{\sa\not\in\calK^n\}]^{\top}$, $\calM_{b^n}$ is a linear MDP under $\wt\phi$.


\begin{claim}[Linear Property of $\calM_{b^n}$ under $\wt\phi$]
The MDP ${\calM}_{b^n}$ is a linear MDP under features $\wt\phi$.
\label{claim:linear_property}
\end{claim}
\begin{proof}
We design a measure $\wt{\mu} = [\mu, \vec{0}]$. We have $P(\cdot |s,a) = \mu \phi\sa = \wt\mu \wt\phi\sa$. Hence, the transition is still linear under $\wt\phi$. Regarding reward, we set $\wt\theta = [\theta^{\top}, 1/(1-\gamma)]^{\top}$.
For $\sa\in\calK^n$, we simply have $\wt\theta \cdot \wt\phi\sa = \theta\cdot \phi\sa$, and for $\sa\not\in\calK^n$, we have $\wt\theta\cdot \wt\phi\sa = \theta\cdot\phi + 1/(1-\gamma) = r\sa + b^n\sa$.  Hence we have new reward functions being linear under $\wt\phi\sa$.
\end{proof}

With this claim, we can now prove \pref{thm:linear_mdp}.

\begin{proof}[Proof of \pref{thm:linear_mdp}]
Note that $\|\wt\mu\| = \|\mu\| = \xi$, and $\|\wt\theta\| \leq \omega + 1/(1-\gamma)$. Note that in the MDP with transition $P$ and reward $r^n$, we have $V_{\max} \leq b^n\sa / (1-\gamma) \leq 1/(1-\gamma)^2$. Hence, for any policy $\pi$, we have $Q^{\pi}_{b^n}\sa = w^{\pi}\cdot \wt\phi\sa$ with $\|w^\pi\| \leq \omega + 1/(1-\gamma) + \xi / (1-\gamma)^2$. We assume that for on-policy fit, we have $W \geq \omega + 1/(1-\gamma) + \xi / (1-\gamma)^2$.

Hence we have shown that for any $n\in [N]$, $\calM_{b^n}$ is a linear MDP under $\wt\phi\sa$, and hence at any iteration $t$ inside episode $n$, we have $Q^t(s,a; r+ b^n)$ is a linear function under feature $\wt\phi\sa$.   This implies that under $\wt\phi\sa$, at episode $n$ and iteration $t$, we have:
\begin{align}
\min_{\theta: \|\theta\| \leq W} \EE_{\sa\sim \rho_\mix^n}\left( \theta\cdot \wt\phi\sa - Q^n_{b^n}\sa    \right)^2 = 0,
\label{eq:linear_regression_linear_mdp}
\end{align} %as the policy cover consists of policies that never visit $a^\dagger$ and 
as there exists $w^t_\star$ with $\|w^t_\star\|\leq W$ such that $Q^n_{b^n}\sa = w^n_\star \cdot \wt\phi\sa$ for all $s$  as $\mathcal{M}_{b^n}$ is a linear MDP with respect to $\widetilde\phi$.%with $a\neq a^\dagger$.





%Recall that three MDPs ($\calM,\calM_{b^n}, \calM^n$) considered in \pref{app:setup_mdps}, and Remark~\pref{remark:relationship_two_mdps}, we have that for any  policy $\pi\in \Pi$  in our policy class, we have $Q^{\pi}_{\calM^n}\sa = Q^\pi(s,a; r+b^n)$, and $A^\pi_{\calM^n}\sa = A^{\pi}(s,a; r+b^n)$ for $a\neq a^\dagger$ as $\pi$ will never pick $a^\dagger$ subsequently. This means that  $Q^\pi_{\calM^n}\sa$ is linear with respect to $\wt\phi\sa$ for $a\neq a^\dagger$.


%This implies that under $\wt\phi\sa$, at episode $n$ and iteration $t$, we have:
%\begin{align}
%\min_{\theta: \|\theta\| \leq W} \EE_{\sa\sim \rho_\mix^n}\left( \theta\cdot \wt\phi\sa - Q^t_{\calM^n}\sa    \right)^2 = 0,
%\label{eq:linear_regression_linear_mdp}
%\end{align} as the policy cover consists of policies that never visit $a^\dagger$ and as there exists $w^t_\star$ with $\|w^t_\star\|\leq W$ such that $Q^t_{b^n}\sa = Q^t_{\calM^n}\sa = w^t_\star \cdot \wt\phi\sa$ for all $s$ with $a\neq a^\dagger$.

This also means  that we can fit advantage function perfectly with the best on-policy fit $w^t_\star$, and hence, we have: %under any state-action pair $\sa$ with $a\neq a^\dagger$:
\begin{align*}
\EE_{\sa \sim d^\star} \left( Q^n\sa - w^n_\star\cdot \widetilde\phi\sa \right)^2 = 0 = \varepsilon_{bias}.
\end{align*}
%\begin{align*}
% A^t(s,a;r+b^n) =  A^{t}_{\Mcal^n}\sa =  w^t_{\star}\cdot \left( \wt\phi\sa - \EE_{a' \sim \pi^t_s} \wt\phi(s,a') \right),
%\end{align*}
%
%
%
%
%
%
%
%
%
%For any comparator $\pi^\star$ in our policy class $\Pi$, we then have:
%\begin{align*}
%\EE_{\sa\sim d^\star}\one\{s\in\calK^n\} \left(  A^t(s,a; r+b^n)-  w^t_{\star} \cdot \left(\wt\phi\sa - \EE_{a'\sim \pi^t_s}\wt\phi(s,a')\right) \right) = 0.
%\end{align*}
%
%
%
%



%
%
%


%
%
%
%
Namely we have shown that \pref{ass:transfer_bias} holds with $\varepsilon_{bias} = 0$. This implies that \pref{lem:variance_bias_n_new} directly holds with $\varepsilon_{bias}= 0$, which implies that \pref{lem:regret_rmax_pg_new} holds with $\varepsilon_{bias} = 0$. Then the rest of the calculation for sample complexity is almost identical to the proof of \pref{thm:detailed_bound_rmax_pg_new} with $\varepsilon_{bias}$ being set to $0$.

%\alekh{Do we have to proceed similarly as the proof, or can we just plug $\varepsilon_{bias} = 0$ in the result?}

This concludes the proof of \pref{thm:linear_mdp}. \end{proof}



==> app_npg_linear_mdp.tex <==
\subsection{Classic NPG for Linear MDPs}

We analyze the performance of a classic NPG using the initial state distribution $\mu_0$ as the reset distribution (i.e., \pref{alg:npg} with $\left(\mu_0, b\sa = 0, \calK = \Scal\times\Acal\right)$ as input). We focus on comparing to a fixed policy $\pi^\star\in\Pi_{linear}$, and denote $d^\star$ as the state-action distribution of $\pi^\star$.

To ensure NPG returns non-vacuous bounds, we first need the following assumption on $\mu_0$.
\begin{assum} Denote $\Sigma_0 := \EE_{s \sim \mu_0, a\sim U(\Acal)}\phi\sa\phi\sa^{\top}$, $\Sigma_\star:= \EE_{s \sim d^\star, a\sim U(\Acal)}\phi\sa\phi\sa^{\top}$, and $\kappa := \tr\left( \Sigma_0^{-1} \Sigma_\star \right)$. We assume $\kappa < \infty$.
%$\kappa_{init}: = \inf_{\sa} \phi\sa^{\top}\Sigma_0 \phi\sa$. We assume $\kappa_{init} > 0$.
\label{asm:init_cond}
\end{assum}
Without this assumption, a direct application of the classic NPG algorithm's guarantee will be vacuous.  Throughout this section, we assume the above assumption holds. 


We first analyze the critic fitting performance.
\begin{lemma}Suppose at episode $n$, we have a policy $\pi^n$, and denote $\theta^n$ as the approximate minimizer of on-policy fit: $\min_{\theta:\|\theta\|\leq W}\EE_{s\sim \mu_0,a\sim U(\Acal)} \left( \theta\cdot \phi^n\sa - Q^{n}\sa \right)^2$ and $Q^n\sa := \theta^n_\star\cdot \phi\sa $. Further assume we have the following property:
\begin{align*}
&\EE_{s\sim \mu_0, a\sim U(\Acal)} \left( Q^n\sa - \theta^n \cdot \phi\sa \right)^2 \leq \varepsilon_{stat};
%\min_{\theta:\|\theta\|\leq W} \EE_{\sa\sim \mu_0} \left(Q^n\sa - \theta\cdot \phi\sa\right)^2 +  \varepsilon_{stat};\\
%& \EE_{\sa\sim d^\star} \left[ A^n\sa - \theta^n_\star\cdot \overline{\phi}^n  \right]  \leq \varepsilon_{bias},
\end{align*} %where $\overline{\phi}^n := \phi\sa - \EE_{a'\sim \pi^n_s} \phi\sa$.
 Then we have:
\begin{align*}
\max_{n\in [N]} V^{n} \geq V^{\pi^\star} - \frac{1}{1-\gamma}\left( 2W\sqrt{\log(A)/ N } + 2A\sqrt{\varepsilon_{stat}  \kappa }\right).
\end{align*}
\label{lemma:NPG_classic}
\end{lemma}
\begin{proof}
From the on-policy fit condition above, we immediately have:
\begin{align*}
\left(\theta^n - \theta^n_\star \right)^{\top} \Sigma_0 \left( \theta^n - \theta^n_\star \right) \leq \varepsilon_{stat}.
\end{align*}
Denote $\widehat{A}^n\sa := \theta^n\cdot \left(\phi\sa - \EE_{a'\sim \pi_s} \phi\sa\right)$.

%First, following the proof of Lemma~\ref{lem:variance_bias_n}, we can show that:
%\begin{align*}
%\EE_{\sa\sim \mu_0}\left( \theta^n_\star \cdot \phi\sa - \theta^n\cdot \phi\sa    \right)^2 \leq \varepsilon_{stats},
%\end{align*}  


%Together with the definitions $\Sigma_0 = \EE_{\sa\sim \mu_0}\phi\sa\phi\sa^{\top}$ and $\kappa_{init} = \sigma_{\min}\left( \Sigma_0 \right)$  this implies that for any $\sa$:
%\begin{align*}
%\left\lvert \phi\sa^{\top} (\theta^n_\star - \theta^n) \right\rvert \leq \| \phi\sa \|_{\Sigma_0^{-1}} \|\theta^n_\star - \theta^n \|_{\Sigma_0} \leq \sqrt{\frac{ {\varepsilon_{stats}} }{\kappa_{init}}}.
%\end{align*}
Now we can bound the prediction error under $d^\star$ as follows:
\begin{align*}
&\EE_{\sa\sim d^\star}\left( A^n\sa - \widehat{A}^n\sa \right) \\
& = \EE_{\sa\sim d^\star}\left( (\theta^n_\star - \theta^n)\cdot \phi\sa \right) + \EE_{s\sim d^\star,a\sim \pi^n}\left( (\theta^n_\star - \theta^n)\cdot \phi\sa \right)\\
& \leq \EE_{\sa\sim d^\star}\left\lvert (\theta^n_\star - \theta^n)\cdot \phi\sa \right\rvert +  \EE_{s\sim d^\star,a\sim \pi^n}\left\lvert (\theta^n_\star - \theta^n)\cdot \phi\sa \right\rvert\\
&\leq A   \EE_{s\sim d^\star,a\sim U(\Acal)}\left\lvert (\theta^n_\star - \theta^n)\cdot \phi\sa \right\rvert +  A\EE_{s\sim d^\star,a\sim U(\Acal)}\left\lvert (\theta^n_\star - \theta^n)\cdot \phi\sa \right\rvert \\
& \leq 2A \sqrt{\varepsilon_{stat}} \sqrt{ \EE_{a\sim d^\star,a\sim U(\Acal)} \phi\sa^{\top} \Sigma_0^{-1} \phi\sa  } \leq 2A\sqrt{\varepsilon_{stat} \tr\left( \Sigma_\star \Sigma_0^{-1} \right)},
%& \leq  \lsqrt{\EE_{\sa\sim d^\star}\left( (\theta^n_\star - \theta^n)\cdot \phi\sa \right)}
%&= \EE_{\sa\sim {d^\star}}\left( A^n\sa - \theta^n_\star\cdot\bar\phi^n \sa \right) + \EE_{\sa\sim {d^\star}}\left( \theta^n_\star \cdot\bar\phi^n\sa - \theta^n\cdot\bar\phi^n\sa \right)\\
%& \leq \varepsilon_{bias} +2\sqrt{ \frac{{\varepsilon_{stats}}}{\kappa_{init}}}.
\end{align*} where the last second inequality uses CS inequality and Jenssen's inequality. 
With this prediction error under $d^\star$, now we can proceed the usual mirror descent analysis for NPG just as we did in the proof of Lemma~\ref{lem:npg_construction}.
Specifically, we will get:
\begin{align*}
\sum_{n=1}^N \EE_{\sa\sim \pi^\star} \left[ \widehat{A}^n\sa \right] \leq \frac{1}{\eta} \kl(\pi^\star_s, \pi^1_s) + \eta TW^2 \leq \log(A)/\eta + \eta T W^2,
\end{align*} which leads to:
\begin{align*}
\sum_{n=1}^N \EE_{\sa\sim d^\star} \left[ \widehat{A}^n\sa \right] \leq 2 W \sqrt{\log(A) N},
\end{align*} with $\eta: = \sqrt{\log(A)/(W^2 N)}$. Using the transfer error of $\widehat{A}^n$ and an application of performance difference lemma, we have:
\begin{align*}
\sum_{n=1}^N (1-\gamma)\left( V^{\pi^\star} - V^n \right) /N \leq 2W\sqrt{\log(A)/ N } + 2A\sqrt{\varepsilon_{stat} \tr\left( \Sigma_\star \Sigma_0^{-1} \right)}.
\end{align*} This concludes the proof.
\end{proof}


\begin{theorem}[Sample Complexity of NPG] Fix $(\epsilon, \delta)$. Under Assumption \pref{asm:init_cond}, we have that with probability at least $1-\delta$, we learned a policy $\hat{\pi}$ such that:
\begin{align*}
V^{\hat\pi} \geq V^\star  - 2 \epsilon,
\end{align*} with total number of samples:
\begin{align*}
\frac{ W^6 A^4 \kappa^2 \nu }{  (1-\gamma)^2 \epsilon^6  },
\end{align*} where $\nu$ contains only log terms and constants $\nu:= 32\log(A) \log\left( 4W^2\log(A)/(\delta\epsilon^2) \right)$.
\label{thm:npg_classic_linear}
\end{theorem}
\begin{proof}
To tolerate $O(\epsilon)$ error,   we need to set $N$ big enough such that $2W\sqrt{\log (A) / N} = \epsilon$. We can verify that $N = \frac{ 4W^2 \log(A) }{\epsilon^2}$ suffices.

Using Lemma~\ref{lem:sgd_dim_free} and a union bound over all episodes $N$, with probability at least $1-\delta$, for any $n\in [N]$, we have:
\begin{align*}
\varepsilon_{stats} \leq \frac{ (2W^2/(1-\gamma)) \sqrt{ \ln(N/\delta)} }{ \sqrt{M} },
\end{align*}
To make $2A \sqrt{\varepsilon_{stats}\kappa} = \epsilon$, it suffices to set $\varepsilon_{stats} =  \frac{\epsilon^2 }{4A^2\kappa} $, which in turn means it suffices to set $M$ as:
\begin{align*}
M = \frac{ 16 W^4 A^4 \kappa^2  \ln(N/\delta)}{ (1-\gamma)^2 \epsilon^4 }.
\end{align*}
The total number of samples will be $NM$, which is at the order:
\begin{align*}
NM = \frac{ 64 W^6 A^4  \kappa ^2 \log(A) \log\left( 4W^2\log(A)/(\delta\epsilon^2) \right) }{  (1-\gamma)^2 \epsilon^6},
\end{align*} which concludes the proof.
\end{proof}



==> app_reward_free.tex <==
\subsection{Application to Reward-free Exploration in Linear MDPs}
\label{app:reward_free_explore}
We can run our algorithm in a reward free setting, i.e., $r\sa = 0$ for all $\sa$. In high level, under reward free setting, \alg tries to explore the entire state-action space as quickly as possible.

For notation simplicity, we focus on linear MDPs in this section (but similar agnostic result can be achieved using the concept of transfer bias).

To do reward-free exploration, we need a slight modification: \alg introduces a termination condition which indicates when we terminate the algorithm (i.e., when we have explored sufficiently except for those state-actions which are hard to reach under any policy). At the end of episode $n$, we check the following termination criteria:
\begin{align}
\label{eq:termination_critera}
\sum_{\sa\not\in\Kcal^n} d^{\pi^{n+1}}\sa \leq \theta \in\mathbb{R}^+,
\end{align} where $\theta$ is some function of accuracy parameter $\epsilon$ and  horizon $(1-\gamma)$ which we will specifiy in the main theorem (\pref{thm:reward_free}) in this section. We terminate if Inequality~\ref{eq:termination_critera} is satisfied and \alg outputs the policy cover $\{\pi^0,\dots, \pi^n \}$. We have the following guarantee for reward free exploration.
\begin{theorem}[Sample Complexity of Reward-free Exploration]
Set the parameters as follows:
\begin{align*}
&\beta = \frac{\epsilon^2(1-\gamma)^2}{4W^2}, \quad M =  \frac{ 576 W^4 \wt{d}^2 \ln(NT/\delta )\ln( 2\wt{d}/(\beta\epsilon(1-\gamma)))^2 }{\epsilon^6(1-\gamma)^{10}},\\
%\varepsilon_{stat} = \frac{(1-\gamma)^3 \epsilon^3}{\widetilde{d}\ln(W^2\widetilde{d} /(\epsilon(1-\gamma)))}, \\
& \theta = (1-\gamma)\epsilon,  \quad \lambda = 1, \quad T = \frac{4W^2 \log(A)}{(1-\gamma)^2 \epsilon^2}.
\end{align*}  With probability at least $1-\delta$, the algorithm terminates within at most $N$ episodes with $N \leq \frac{4\widetilde{d}}{\beta\theta}\log\left(\frac{4\widetilde{d}}{\lambda \beta\theta}\right)$, and upon termination, we identify a set of hard-to-reach state action pairs, i.e., $\overline\Kcal^N := \Scal\times\Acal \setminus \Kcal^N$, such that:
\begin{align*}
\max_{\pi\in\Pi_{linear}} \sum_{\sa \in \overline{\Kcal}^N} d^{\pi}\sa \leq  4\epsilon,
\end{align*}  with total number of samples:
\begin{align*}
\frac{c \nu W^8 \wt{d}^3 \ln(A)}{\epsilon^{11}(1-\gamma)^{15}},
\end{align*} where $c $ is a universal constant, and $\nu$ contains only log terms:
\begin{align*}
\nu & = \ln\left(\frac{W^2\wt{d}}{\epsilon^3 (1-\gamma)^3}\right)\ln\left(\frac{\wt{d} W^4\ln(A) }{\epsilon^5(1-\gamma)^5\delta} \ln\left( \frac{2\wt{d}W^2}{\epsilon^3(1-\gamma)^3} \right)\right) \ln^2\left(  \frac{W^2\wt{d}}{\epsilon^3(1-\gamma)^3} \right)\\
& \qquad + \ln^3\left( \frac{W^2 \wt{d}}{\epsilon^3(1-\gamma)^3} \right) \ln\left( \frac{ \wh{d}\wt{d}  }{ \epsilon^3(1-\gamma)^3\delta}\ln\left( \frac{W^2\wt{d}}{\epsilon^3(1-\gamma)^3} \right) \right).
\end{align*}
\label{thm:reward_free}
\end{theorem}

The benefit of reward-free exploration is that once exploration is done, one can efficient optimize any given reward functions.
The next theorem shows that with the policy cover from \alg, for any future non-zero reward we could have, we can run the classic NPG with the policy cover's induced state-action distribution as reset/initial distribution to achieve a near optimal policy.
\begin{theorem}[Post NPG optimization with the Policy Cover from \alg]
Conditioned on \pref{thm:reward_free} holding, for the policy cover (denote $\rho^N_{\mix} = \frac{1}{N} \sum_i d^{\pi^i}$), given any non-zero reward $r'\sa\in [0,1]$, run NPG (\pref{alg:npg}), with $(\rho^N_{\mix}, b^N\sa = 0,\forall\sa)$ as inputs, with parameters:
\begin{align*}
T = 4W^2 \log(A)/\epsilon^2, \quad M =   \frac{ 576 W^4 \wt{d}^2 \ln(NT/\delta )\ln( 2\wt{d}/(\beta\epsilon(1-\gamma)))^2 }{\epsilon^6(1-\gamma)^{10}}.
\end{align*} Then with probability at least $1-\delta$, \pref{alg:npg} outputs a policy $\hat{\pi}$ such that:
\begin{align*}
\EE\left[\sum_{t}\gamma^t r'(s_t,a_t) | \hat{\pi}, s_0\sim \mu_0\right] \geq \max_{\pi\in\Pi_{linear}}\EE\left[\sum_{t}\gamma^t r'(s_t,a_t) | {\pi}, s_0\sim \mu_0\right]   - O\left(\frac{ \epsilon }{(1-\gamma)^2} + \frac{W\epsilon}{1-\gamma}\right),
\end{align*} with total number of samples
\begin{align*}
O\left(\frac{ W^6 \log(A) \wt{d}^2 }{\epsilon^8(1-\gamma)^{10}}  \ln(NT/\delta )\ln( 2\wt{d}/(\beta\epsilon(1-\gamma)))^2 \right).
\end{align*}
%$\widetilde{O}\left(\frac{W^6 \nu}{(1-\gamma)^2 \epsilon^6}\right)$.
%For the policy cover, denote $\Sigma^N_{cov} = \frac{1}{N} \sum_{i=1}^N \Sigma^i $.
%where for state-action that is not hard to reach, i.e., $\sa\not\in\overline\Kcal$, we have a policy cover $\{\pi^1,\dots, \pi^N\}$ which allows us to do accurate on-policy fitting for any given policy $\pi$, measured under any comparator's distribution, i.e.,
%\begin{align*}
%\EE_{\sa\sim d^\star_{linear}} A^{\pi}
%\end{align*}
%such that:
%\begin{align*}
%\phi\sa^{\top} \left(\Sigma^N_{\mix}\right)^{-1} \phi\sa \leq \beta := \frac{ \epsilon^2 (1-\gamma)^2 }{ 4W^2 }.
%\end{align*}
\label{thm:reward_free_npg_opt}
\end{theorem}

The above theorem indicates that once a reward-free phase is done, \alg identifies a hard-to-reach state-action subspace, and a policy cover which can be used as the reset distribution for NPG for any new given reward functions. Note that unlike prior results for NPG~\citep{geist2019theory,agarwal2019optimalityshani2019adaptive}, this is a global optimality guarantee without any distribution mismatch or concetrability coefficients since we have provided the algorithm with a favorable initial distribution from the reward-free exploration phase.


\subsubsection{Proof of \pref{thm:reward_free} and \pref{thm:reward_free_npg_opt}}
To prove the above main theorem, we first show that the algorithm will terminate with finite number of bounds.

%At the end of the $n$-th episode, we terminate our algorithm if $\sum_{\sa\not\in\Kcal^n} d^{\pi^{n+1}}\sa \leq \theta\in\mathbb{R}^+$ with some pre-defined threshold $\theta$.

\begin{lemma}[Total Number of Episodes]
Assume that for $n = 0,\dots N $, we have $\sum_{\sa\not\in\Kcal^n}\sa  \geq \theta$ (i.e., algorithm does not terminate), we must have:
\begin{align*}
N \leq  \frac{4\widetilde{d}}{\beta\theta} \log\left( \frac{4\widetilde{d}}{\lambda \beta\theta} \right).
\end{align*}
\end{lemma}
\begin{proof}Based on the proof of \pref{lem:potential_argument_n}, we have that:
\begin{align*}
&\sum_{n=1}^N \beta \theta \leq \beta \EE_{\sa\sim d^{n+1}}\one\{\sa\not\in\Kcal^n\} \leq \sum_n \tr\left(\Sigma^{n+1} \left( \Sigma^n_{\mix}\right)^{-1}\right) \\
&\leq 2\log\det\left( \Sigma^N_{\mix} \right) \leq 2\widetilde{d} \log\left(N/\lambda + 1\right).
\end{align*} which implies that:
\begin{align*}
N \leq \frac{2\widetilde{d}}{ \beta\theta}\log\left( N / \lambda + 1\right).
\end{align*} This concludes the proof.
\end{proof}





Now we can prove the main theorem below.
\begin{proof}[Proof of \pref{thm:reward_free}]
Focus on the last iteration $N$ where the algorithm terminates. Using \pref{lem:perf_absorb}, we have that:
\begin{align*}
V^{N+1}_{\mathcal{M}^{N}} \leq V^{{N+1}}_{\mathcal{M}} + \frac{1}{1-\gamma} \sum_{\sa\not\in\Kcal^N} d^{N+1}\sa \leq V^{N+1}_{\mathcal{M}} + \frac{\theta}{1- \gamma} = \frac{\theta}{1-\gamma},
\end{align*} where the second inequality uses the termination criteria and the last equality uses the fact that $V^\pi_{M} = 0$ for any $\pi$ as $r\sa = 0$ for all $\sa$.

Recall the definition of $\mathcal{M}^N$ from Item~\ref{item:mdp_3} and the NPG guarantee, we have for any comparator $\widetilde\pi$:
\begin{align*}
V^{\widetilde\pi^{N}}_{\mathcal{M}^N}  - \frac{1}{1-\gamma}\left( 2W\sqrt{\frac{\log(A)}{T}}  + 2\sqrt{\beta \lambda W^2 } + 2\sqrt{\beta N \varepsilon_{stat}} \right) \leq V^{N+1}_{\mathcal{M}^N} \leq \frac{\theta}{1-\gamma}.
\end{align*}

To link the above results to the maximum possible escaping probability, we define another MDP $\widetilde{\mathcal{M}}$ such that $\widetilde{\mathcal{M}}$ and $\mathcal{M}$ has the same transition dynamics, but $\widetilde{\mathcal{M}}$ has rewards $r(s,a) = 1$ for $\sa\not\in\Kcal^N$ and $r(s,a) = 0$ otherwise. We also construct the ``absorbing'' MDP $\widetilde{\mathcal{M}}^N$ analogous of $\mathcal{M}^n$ to $\mathcal{M}$. Note that for any policy $\widetilde{\pi}$, we have:
\begin{align*}
V^{\widetilde\pi}_{\widetilde{\mathcal{M}}} = \sum_{\sa\not\in\Kcal^N}  d^{\widetilde\pi}\sa, \quad V^{\widetilde{\pi}^N}_{\widetilde{\mathcal{M}}^N} \geq V^{\widetilde\pi}_{\widetilde{\mathcal{M}}}.
\end{align*}
Note that $V^{\tilde\pi^N}_{\widetilde{\mathcal{M}}^N} = V^{\widetilde{\pi}^N }_{{\mathcal{M}}^N}$, since $\widetilde\pi^N$ only picks $a^{\dagger}$ at $s\not\in\Kcal^N$ and ${\mathcal{M}}^N$ and $\widetilde{\mathcal{M}}^N$ only differ at $\sa\not\in\Kcal^N$ in terms of rewards.

Combine the above results, we get:
\begin{align*}
&\sum_{\sa\not\in\Kcal^N} d^{\widetilde\pi}\sa = V^{\widetilde\pi}_{\widetilde{\mathcal{M}}} \leq V^{\widetilde\pi^N}_{\widetilde{\mathcal{M}}^N} = V^{\widetilde\pi^N}_{\mathcal{M}^N} \\
& \leq  \frac{1}{1-\gamma}\left( 2W\sqrt{\frac{\log(A)}{T}} + 2\sqrt{\beta \lambda W^2 } + 2\sqrt{\beta N \varepsilon_{stat}} \right)+ \frac{\theta}{1-\gamma}.
\end{align*}
Take $\widetilde\pi = \arg\max_{\pi\in\Pi_{linear}} \sum_{\sa\not\in\Kcal^N} d^{\pi}\sa$ and set parameters based on the values proposed in the main theorem, we conclude that:
\begin{align*}
\max_{\pi\in\Pi_{linear}} \sum_{\sa\not\in\Kcal^N} d^\pi\sa \leq 4\epsilon.
\end{align*}

Now we calculate the sample complexity.  Following the proof of \pref{thm:detailed_bound_rmax_pg}, we have that the total number of samples one use for constructing $\widehat\Sigma^n_{\mix}$ is:
\begin{align*}
%\label{eq:source_1}
&N \times \left(N^2 \ln\left( \wh{d} N /\delta \right)\right)  = N^3 \ln\left( \wh{d} N /\delta \right)
%&= \frac{8\wt{d}^3 W^6}{ \epsilon^9(1-\gamma)^{9}}\ln^3\left( \frac{8W^2 \wt{d}}{\epsilon^3(1-\gamma)^3} \right) \ln\left( \frac{ 2\wh{d}\wt{d}  }{ \epsilon^3(1-\gamma)^3\delta}\ln\left( \frac{8W^2\wt{d}}{\epsilon^3(1-\gamma)^3} \right) \right)\\
 =  \frac{c_1 \nu_1 \widetilde{d}^3 W^6}{\epsilon^9(1-\gamma)^9},
\end{align*} where $c_1$ is a  constant and $\nu_1$ contains log-terms $\nu_1:= \ln^3\left( \frac{8W^2 \wt{d}}{\epsilon^3(1-\gamma)^3} \right) \ln\left( \frac{ 2\wh{d}\wt{d}  }{ \epsilon^3(1-\gamma)^3\delta}\ln\left( \frac{8W^2\wt{d}}{\epsilon^3(1-\gamma)^3} \right) \right)$.

The second source of sample complexity comes from on-policy fit. To derive $\varepsilon_{stat} = (1-\gamma)^3 \epsilon^3 / \widetilde{d}$, we need to set $M$ (the number of samples for on-policy fit in each iteration $t$ and episode $n$):
\begin{align*}
M =  \frac{ 576 W^4 \wt{d}^2 \ln(NT/\delta )\ln( 2\wt{d}/(\beta\epsilon(1-\gamma)))^2 }{\epsilon^6(1-\gamma)^{10}}
\end{align*}
Considering every episode $n\in [N]$ and every iteration $t\in [T]$, we have the total number of samples needed for NPG is:
\begin{align*}
NT \cdot M  %& = \frac{ 8 W^2 \wt{d} }{\epsilon^3 (1-\gamma)^3}\ln\left( \frac{8W^2\wt{d}}{\epsilon^3 (1-\gamma)^3} \right) \times \frac{4W^2 \log(A)}{(1-\gamma)^2 \epsilon^2} \times  \frac{ 576 W^4 \wt{d}^2 \ln(NT/\delta )\ln( 2\wt{d}/(\beta\epsilon(1-\gamma)))^2 }{\epsilon^6(1-\gamma)^{10}}\\
%& =  \frac{c_2 W^8 \wt{d}^{3} \ln(A) }{ \epsilon^{11}(1-\gamma)^{15} } \ln\left(\frac{W^2\wt{d}}{\epsilon^3 (1-\gamma)^3}\right)\ln\left(\frac{\wt{d} W^4\ln(A) }{\epsilon^5(1-\gamma)^5\delta} \ln\left( \frac{2\wt{d}W^2}{\epsilon^3(1-\gamma)^3} \right)\right) \ln^2\left(  \frac{W^2\wt{d}}{\epsilon^3(1-\gamma)^3} \right) \\
%& = \frac{c_2 \nu_2 W^8 \wt{d}^{3} \ln(A) }{ \epsilon^{11}(1-\gamma)^{15} },
%\end{align*} where $c_2$ is a positive universal constant, and $\nu_2$ only contains log terms:
%\begin{align*}
%\nu_2 = \ln\left(\frac{W^2\wt{d}}{\epsilon^3 (1-\gamma)^3}\right)\ln\left(\frac{\wt{d} W^4\ln(A) }{\epsilon^5(1-\gamma)^5\delta} \ln\left( \frac{2\wt{d}W^2}{\epsilon^3(1-\gamma)^3} \right)\right) \ln^2\left(  \frac{W^2\wt{d}}{\epsilon^3(1-\gamma)^3} \right).
%\end{align*}
%Combine two sources of samples, we have that the total number of samples is bounded as:
%\begin{align*}
%\frac{c_2 \nu_2 W^8 \wt{d}^{3} \ln(A) }{ \epsilon^{11}(1-\gamma)^{15} } +  \frac{c_1 \nu_2 \wt{d}^3 W^6}{ \epsilon^9(1-\gamma)^{9}},
\end{align*}
The rest of the caculation involves subistituing $M, N, T$ into the above expression and then combining two sources of samples together, exactly as what we did for the proof of \pref{thm:detailed_bound_rmax_pg} .
\end{proof}

Now once the learned the policy cover, given any non-zero reward $r\sa$, and any policy $\pi$, we can also show that by leveraging the policy cover we have upon termination, we can accurately estimate any policy's advantage on any state-action pair in the known set $\Kcal^N$ using the fact that for any $\sa\in\calK^n$, we have $\phi\sa^{\top}\left(\Sigma^N_{\mix}\right)^{-1}\phi\sa \leq \beta$.
\begin{lemma}[Policy Cover For On-Policy Critic Fit]
Denote the policy cover's induced state-action distribution as $\rho^N_{\mix} = \frac{1}{N} \sum_i d^{\pi^i}$. Given any non-zero reward $r\sa\in [0,1]$, and any policy $\pi$, denote $\hat\theta$ as the approximate minimizer of $\EE_{\sa\sim \rho^N_{\mix}}\left( \theta\cdot \phi\sa - Q^{\pi}\sa  \right)^2$, i.e., $\EE_{\sa\sim \rho^N_{\mix}}\left( \hat\theta\cdot \phi\sa - Q^{\pi}\sa  \right)^2 \leq \varepsilon_{stat}$. We have that for any comparator $\widetilde\pi$:
\begin{align*}
\EE_{\sa\sim d^{\widetilde\pi}}\left( A^{\pi}\sa - \hat\theta\cdot\overline{\phi}\sa \right)\one\{\sa\in\Kcal^N\} \leq 2\sqrt{\beta \lambda W^2 } + 2\sqrt{\beta  N \varepsilon_{stat}},
\end{align*} where $\overline\phi\sa = \phi\sa - \EE_{a'\sim \pi_s}\phi(s,a')$.
%running classic NPG (\pref{alg:npg} with $(\rho^N_{\mix}, b= 0, \Kcal = \Kcal^N)$ as inputs) with $\rho^N_\mix$ as the reset distribution to optimize with respect to $r'$
\label{lem:policy_cover_fit}
\end{lemma}
\begin{proof}
Denote $Q^\pi\sa:= \theta_\star\cdot \phi\sa$. For any state-action pair in $\Kcal^N$, following the similar derivation we have in the proof of \pref{lem:variance_bias_n}, we thus have:
\begin{align*}
\left\lvert \phi\sa \cdot \left( \theta_\star - \hat\theta  \right) \right\rvert \leq \sqrt{\beta \lambda W^2 } + \sqrt{\beta N \varepsilon_{stat}}, \quad \forall \sa\in\Kcal^N.
\end{align*}
As the above bound is state-action wise, thus for any policy distribution $d^{\widetilde\pi}$, for $A^\pi$, we have that:
\begin{align*}
&\EE_{\sa\sim d^{\widetilde\pi}} \left( A^\pi\sa - \hat\theta\cdot \overline\phi\sa  \right)\one\{\sa\in \Kcal^N\} \leq2\sqrt{\beta \lambda W^2 } + 2\sqrt{\beta N \varepsilon_{stat}}.
\end{align*}%where $\varepsilon'_{bias} = \EE_{\sa\sim d^\star}\left( A'\sa - \theta_\star\cdot \overline\phi\sa \right)$.
This concludes the proof.
\end{proof}


\begin{proof}[Proof of \pref{thm:reward_free_npg_opt}]
Now for the performance of NPG on a new reward function $r'$ with $\rho_{\mix}^N$ as the reset distribution,  from \pref{lem:policy_cover_fit}, we have that for any $\pi^t$ generated during the NPG's run, we have:
\begin{align*}
\EE_{\sa\sim d^{\star}}\left( A^{t}\sa - \hat\theta^t \cdot\overline{\phi}^n\sa \right)\one\{\sa\in\Kcal^N\} \leq 2\sqrt{\beta \lambda W^2 } + 2\sqrt{\beta  N \varepsilon_{stat}}.
\end{align*}
With a performance difference lemma application, we have:
\begin{align*}
&V^{\pi^\star} - V^{\pi^t} = \frac{1}{1-\gamma}\EE_{\sa\sim d^{\star}} A^{t}\sa \\
& = \frac{1}{1-\gamma}\EE_{\sa\sim d^{\star}} A^{t}\sa \one\{\sa\in\Kcal^N\} + \frac{1}{1-\gamma}\EE_{\sa\sim d^{\star}} A^{t}\sa\one\{\sa\not\in\Kcal^N\}\\
& \leq \frac{1}{1-\gamma}\EE_{\sa\sim d^{\star}} A^{t}\sa \one\{\sa\in\Kcal^N\} +  \frac{4\epsilon}{(1-\gamma)^2} \\
& \leq \frac{1}{1-\gamma}\EE_{\sa\sim d^{\star}} \widehat{A}^{t}\sa \one\{\sa\in\Kcal^N\} +  \frac{4\epsilon}{(1-\gamma)^2}  + \frac{2\sqrt{\beta \lambda W^2 } + 2\sqrt{\beta  N \varepsilon_{stat}}}{1-\gamma}
\end{align*} where we use $\max_{\pi} \EE_{\sa\sim d^{\pi}} \one\{\sa\not\in\Kcal^N\} \leq \epsilon$ (recall $\overline{\Kcal}^N := \Scal\times\Acal \setminus \Kcal^N$).
As NPG is performing the following update rule,
\begin{align*}
\pi^{t+1}(\cdot |s) \propto \pi^t(\cdot | s)  \exp\left(\eta \widehat{A}^t \sa \right),
\end{align*} with a Mirror Descent analysis, we have:
\begin{align*}
\sum_{t=1}^{T} \EE_{a\sim \pi^\star_s} \widehat{A}^t\sa \leq 2W \sqrt{\log(A) T }.
\end{align*}
Add expectation with respect to $d^\star$ on both sides, we get:
\begin{align*}
\sum_{t=1}^T \EE_{\sa\sim d^\star} \widehat{A}^t\sa = \sum_{t=1}^T \EE_{\sa\sim d^\star} \widehat{A}^t\sa\one\{\sa\in\calK^n \} + \sum_{t=1}^T \EE_{\sa\sim d^\star} \widehat{A}^t\sa\one\{\sa\not\in\calK^N\}
\end{align*} which implies that:
\begin{align*}
&\sum_{t=1}^T \EE_{\sa\sim d^\star} \widehat{A}^t\sa\one\{\sa\in\calK^n \}  \leq 2W\sqrt{\log(A)T} - \sum_{t=1}^T \EE_{\sa\sim d^\star} \widehat{A}^t\sa\one\{\sa\not\in\calK^N\} \\
& \leq 2W\sqrt{\log(A) T} + T\epsilon \max_{s,a} | \widehat{A}^t\sa | \leq  2W\sqrt{\log(A)T} + TW \epsilon.
\end{align*}
This leads to the following result:
\begin{align*}
\sum_{t} \left(V^{\pi^\star} - V^{\pi^t}\right)/T  \leq \frac{1}{1-\gamma}\left(  2W\sqrt{\log(A)/T}  + \frac{4\epsilon}{(1-\gamma)}  + W\epsilon + {2\sqrt{\beta \lambda W^2 } + 2\sqrt{\beta  N \varepsilon_{stat}}}\right),
\end{align*} where we abuse the notation a bit by denoting $V^{\pi}$ as the expected total reward of $\pi$ under the new reward function $r'$.
With $T:= 4W^2\log(A)/\epsilon^2$, and the values of $\beta, \lambda, M, \varepsilon_{stat}$ defined in \pref{thm:reward_free}, we can simply the above inequality to:
\begin{align*}
\sum_{t} \left(V^{\pi^\star} - V^{\pi^t}\right)/T  \leq O\left( \frac{\epsilon}{(1-\gamma)^2} + \frac{W\epsilon}{1-\gamma}\right).
\end{align*}
The total number of samples one needs is:
\begin{align*}
&M \cdot T  =  \frac{ 576 W^4 \wt{d}^2 \ln(NT/\delta )\ln( 2\wt{d}/(\beta\epsilon(1-\gamma)))^2 }{\epsilon^6(1-\gamma)^{10}} \frac{4W^2\log(A)}{\epsilon^2} \\
& =  \frac{ 2304 W^6 \log(A) \wt{d}^2 \ln(NT/\delta )\ln( 2\wt{d}/(\beta\epsilon(1-\gamma)))^2 }{\epsilon^8(1-\gamma)^{10}}
\end{align*}
This concludes the proof.
\end{proof}


==> app_state_act_aggregation.tex <==
%!TEX root = main.tex

\section{Application to State-Aggregation (\pref{thm:state_aggregation})}
\label{app:state_agg}

%In this section, we analyze \pref{thm:state_aggregation} for state-aggregation.  Similarly, we leverage the general theorem~\ref{thm:detailed_bound_rmax_pg} and bound the transfer error using aggregation errors.

In this section, we analyze \pref{thm:state_aggregation} for state-aggregation. Different from the Linear MDP case where it is required to change the critic fitting procedure, we do not need to perform any modification of algorithm here. Hence, we are going to leverage the general theorem~\ref{thm:detailed_bound_rmax_pg} and bound the transfer bias  $\epsilon_{bias}$ using aggregation errors .


First recall the definition of state aggregation $\phi:\mathcal{S}\times\mathcal{A} \to\mathcal{Z}$. We abuse the notation a bit, and denote $\phi\sa = \one\{\phi\sa = z\} \in\mathbb{R}^{|\mathcal{Z}|}$, i.e., the feature vector $\phi$ indicates which $z$ the state action pair $\sa$ is mapped to.  The following claim reasons the approximation of $Q$ values under state aggregation.
\begin{claim} \label{claim:state_agg} Denote aggregation error $\epsilon_{z}$ as:
\begin{align*}
\max\left\{ \| P(\cdot | s,a) - P(\cdot | s', a') \|_1, \lvert r(s,a) - r(s',a') \rvert \right\} \leq \epsilon_{z}, \forall \sa,(s',a'), \text{ s.t., } \phi\sa = \phi(s',a') = z.
\end{align*} Then, for any policy $\pi$, $\sa,(s',a'), z$, such that $\phi(s,a) = \phi(s',a') = z$, we have:
\begin{align*}
\left\lvert Q^{\pi}(s, a) - Q^{\pi}(s', a')\right\rvert \leq  \frac{r_{\max} \epsilon_{z} }{1-\gamma},
\end{align*} where $r\sa\in [0, r_{\max}]$ for $r_{\max}\in \mathbb{R}^+$.
\end{claim}
\begin{proof}
Starting from the definition of $Q^{\pi}$, we have:
\begin{align*}
&\left\lvert Q^{\pi}(s, a) - Q^{\pi}(s', a')\right\rvert = \lvert r(s,a) - r(s' ,a') \rvert + \gamma \lvert \EE_{x'\sim P_{s,a}} V^{\pi}(s') - \EE_{x'\sim P_{s',a'}} V^{\pi}(s')  \rvert \\
& \leq \epsilon_{z} + \frac{r_{\max}\gamma}{1-\gamma} \left\| P_{s,a} - P_{s',a'} \right\|_1 \leq \frac{r_{\max}\epsilon_{z}}{1-\gamma},
\end{align*} where we use the assumption that $\phi(s,a) = \phi(s',a') = z$, and the fact that value function $\|V\|_{\infty} \leq r_{\max}/(1-\gamma)$ as $r\sa\in [0, r_{\max}]$.
\end{proof}

Recall the definition $\epsilon_{misspec}(z) = \epsilon_{z}$ and we also denote the $\ell_\infty$ error as $\epsilon_{misspec} := \max_{z} \epsilon_{misspec}(z)$.

Now we can bound the transfer error defined in \pref{ass:transfer_bias}.
%We leverage the general result in \pref{thm:detailed_bound_rmax_pg} to prove \pref{thm:state_aggregation} by giving a specific bound on $\varepsilon_{bias}$.

\begin{lemma}[Bounding Transfer error] Consider an arbitrary comparator $\pi^\star$ with $d^{\star}(s,a) := d^{\pi^\star}(s) \text{Unif}_{\Acal}(a)$.
Throughout \alg, consider any episode $n$, we have:
\begin{align*}
\EE_{\sa \sim d^\star}\left( Q^n(s,a; r+b^n) - \theta^n_\star\sa  \right)^2 \leq \frac{\EE_{\sa\sim d^\star} [\epsilon^2_{misspec}(\phi\sa)] }{ (1-\gamma)^4},
\end{align*} %where $A^t_\star\sa = \theta^t_\star\cdot \phi\sa - \EE_{a'\sim \pi^t_s} \theta^t_\star\cdot \phi(s,a')$, 
where $\theta^t_\star$ is one of the best on-policy fit:
\begin{align*}
\theta^t_\star \in \arg\min_{\|\theta\|\leq W}\EE_{ \sa\sim \rho^n_{\mix}} \left(\theta\cdot\phi\sa - Q^n(s,a; r+b^n)\right)^2.
\end{align*}\label{lem:bias_in_state_agg}
\end{lemma}
\begin{proof}
Recall that notation $Q^n_{b^n}\sa$ is in short of $Q^n(s,a; r+b^n)$.
First note that as $b^n\sa \in [0,1/(1-\gamma)]$, we must have $Q^n_{b^n}\sa \in [1, 1/(1-\gamma)^2]$.  Second, for any $s,a$ such that $\phi\sa = \phi(s',a') = z$,  we have $\phi(s,a) = \phi(s',a')$ which means that $\sa\in \Kcal^n$ if and only if $(s',a')\in\Kcal^n$ as their features are identical.  This means that the reward misspecification assumption still holds under model $\mathcal{M}_{b^n}$, i.e., $\lvert r(s,a) + b^n(s,a) - r(s',a') - b^n(s',a') \rvert \leq \epsilon_{z}$.

Now let us consider $\theta^t_{\star}$. Using the definition of the state aggregation, we have:
\begin{align*}
&\EE_{ \sa\sim \rho^n_{\mix}} \left(\theta\cdot\phi\sa - Q^n_{b^n}\sa\right)^2 \\
&= \EE_{\sa\sim \rho^n_{\mix}} \sum_{z} \one\{\phi(s,a) = z\} \left( \theta_{z} - Q^n_{b^n}\sa \right)^2,
%& = \EE_{}
\end{align*} which means that for $\theta^t_{\star}$, we have:
\begin{align*}
\sum_{s,a} \rho^n_{\mix}(s,a) \one\{\phi(s,a) = z\} \left( \theta_{z} - Q^n_{b^n}(s,a)\right) = 0,
\end{align*} which implies that $\theta^t_{\star, z} := \frac{  \sum_{s,a} \rho^n_{\mix}(s,a)\one\{\phi(s,a) = z\}  Q^n_{b^n}(s,a)}{ \sum_{s,a}\rho^n_{\mix}(s,a)\one\{\phi(s,a) = z\} } $.
Hence, for any $s'',a'' $ such that $\phi(s'',a'') = z$, we must have:
\begin{align*}
&\left\lvert \theta_{\star, z} - Q^{n}_{b^n}(s'', a'') \right\rvert \\
& = \left\lvert  \frac{  \sum_{s,a} \rho^n_{\mix}(s,a)\one\{\phi(s,a) = z\}  Q^n_{b^n}(s,a)}{ \sum_{s,a}\rho^n_{\mix}(s,a)\one\{\phi(s,a) = z\} }  - Q^n_{b^n}(s'',a'')  \right\rvert\\
& = \left\lvert  \frac{\sum_{s,a} \rho^n_{\mix}(s,a)\one\{\phi(s,a) = z\} \left( Q^n_{b^n}(s,a) - Q^n_{b^n}(s'',a'') \right)}{ \sum_{s,a}\rho^n_{\mix}(s,a)\one\{\phi(s,a) = z\} }         \right\rvert
%& \leq \left\vert  \frac{  \sum_{s,a'} \rho^n_{\mix}(s,a')\one\{\phi(s) = z, a' = a\}  Q^n_{b^n}(s'',a)}{ \sum_{s,a'}\rho^n_{\mix}(s,a')\one\{\phi(s) = z, a'= a\} }  -  Q^{n}_{b^n}(s'', a)  \right\rvert \\
%& \qquad + \left\lvert   \frac{  \sum_{s,a'} \rho^n_{\mix}(s,a')\one\{\phi(s) = z, a' = a\}  (Q^n_{b^n}(s'',a)  - Q^n_{b^n}(s,a))}{ \sum_{s,a'}\rho^n_{\mix}(s,a')\one\{\phi(s) = z, a'= a\} }     \right\rvert \\
 \leq \frac{\epsilon_{z}}{ (1-\gamma)^2  },
\end{align*} where we use Claim~\ref{claim:state_agg}.

%\alekh{I don't follow the additional $1/(1-\gamma)$ factor here? It seems like you plugin C.10 directly and since the bonus is identical in the $s,a$ and $s'',a$ as you show above, there is no blowup by any factors?}

%\begin{align*}
%\theta^t_{\star, z,a} =  \EE_{s\sim \rho^n_{\mix}} \one\{\phi(s) = z\} Q^t_{b^n}\sa,
%\end{align*}
Note $|\theta^n_{\star,z}| \leq \frac{1}{(1-\gamma)^2}$ and $\|\theta^n_\star\|_2 \leq \sqrt{\frac{Z}{(1-\gamma)^4}} := W$ in this case.%\alekh{There is some $\ell_2$ versus $\ell_\infty$ confusion here?}

Now for any state-action distribution $d$, we will have:
\begin{align}
&\EE_{\sa\sim d} \left(Q^n_{b^n}\sa -\theta^n_\star\cdot \phi\sa \right)^2 \nonumber \\
& = \sum_{z} \EE_{\sa\sim d} \one\{\phi(s,a) = z\} \left( Q^n_{b^n}(s,a) - \theta^n_{\star,z} \right)^2 \nonumber\\
& \leq \EE_{(z)\sim d} \frac{\epsilon_{z}^2}{(1-\gamma)^4} \nonumber \leq \frac{\EE_{z\sim d} \epsilon_{misspec}(z)^2 }{(1-\gamma)^4} = \frac{\EE_{\sa\sim d}\left[ \epsilon_{misspec}(\phi(s,a))^2\right] }{(1-\gamma)^4}.
\end{align} %where $\epsilon_{misspec}(z) = \max_{a} \epsilon_{z,a}$.


\end{proof}






The above lemma (\pref{lem:bias_in_state_agg}) essentially proves that transfer error $\epsilon_{bias} = \frac{\EE_{z\sim d^\star} [\epsilon_{misspec}^2(z)] }{ (1-\gamma)^4 }$.

Now call \pref{thm:detailed_bound_rmax_pg} with $\epsilon_{bias} = \frac{\EE_{z\sim d^\star_{}} [\epsilon^2_{misspec}(z)] }{ (1-\gamma)^4 }$, we conclude the proof of \pref{thm:state_aggregation}. 
\qed


\iffalse
\subsection{Application to Mis-specified Linear MDPs}
We consider model mis-specification in linear MDPs, which is defined formally as follows.
\begin{align*}
P(s' | s,a) = \mu(s') \phi\sa + \epsilon_{s,a}, \quad r(s,a) = \theta\cdot\phi\sa + \epsilon_{s,a},
\end{align*} for some $\epsilon_{s,a}\in [0,1]$ for all $\sa$.

The following claim shows that the resulting $Q^{\pi}$ for any policy $\pi$ is approximately linear. 
\begin{claim}Consider any policy $\pi$, and any reward function $r\sa\in [0, r_{\max}]$. For $Q^{\pi}(\cdot,\cdot; r)$, there exists $\theta^\pi$ such that:
\begin{align*}
\left\lvert Q^\pi(s,a; r) - \theta^\pi \cdot \phi\sa  \right\rvert \leq  \quad \forall \sa.
\end{align*}
\end{claim}
\begin{proof}
to do..
\end{proof}

Consider episode $n$ and the augmented feature $\widetilde\phi\sa = [\phi\sa^{\top}, \one\{\sa\not\in\Kcal^n\}]^{\top}$. 
\fi







==> app_state_aggregation.tex <==
%!TEX root = main.tex

\subsection{Application to State-Aggregation (\pref{thm:state_aggregation})}
\label{app:state_agg}

In this section, we analyze \pref{thm:state_aggregation} for state-aggregation.  Similarly, we leverage the general theorem~\ref{thm:detailed_bound_rmax_pg_new} and bound the transfer error using aggregation errors.

First recall the definition of state aggregation $\phi:\mathcal{S}\times\mathcal{A} \to\mathcal{Z}$. We abuse the notation a bit, and denote $\phi\sa = \one\{\phi\sa = z\} \in\mathbb{R}^{|\mathcal{Z}|}$, i.e., the feature vector $\phi$ indicates which $z$ the state action pair $\sa$ is mapped to.  The following claim reasons the approximation of $Q$ values under state aggregation.
\begin{claim} \label{claim:state_agg} Denote aggregation error $\epsilon_{z}$ as:
\begin{align*}
\max\left\{ \| P(\cdot | s,a) - P(\cdot | s', a') \|_1, \lvert r(s,a) - r(s',a') \rvert \right\} \leq \epsilon_{z}, \forall \sa,(s',a'), \text{ s.t., } \phi\sa = \phi(s',a') = z.
\end{align*} Then, for any policy $\pi$, $\sa,(s',a'), z$, such that $\phi(s,a) = \phi(s',a') = z$, we have:
\begin{align*}
\left\lvert Q^{\pi}(s, a) - Q^{\pi}(s', a')\right\rvert \leq  \frac{r_{\max} \epsilon_{z} }{1-\gamma},
\end{align*} where $r\sa\in [0, r_{\max}]$ for $r_{\max}\in \mathbb{R}^+$.
\end{claim}
\begin{proof}
Starting from the definition of $Q^{\pi}$, we have:
\begin{align*}
&\left\lvert Q^{\pi}(s, a) - Q^{\pi}(s', a')\right\rvert = \lvert r(s,a) - r(s' ,a') \rvert + \gamma \lvert \EE_{x'\sim P_{s,a}} V^{\pi}(s') - \EE_{x'\sim P_{s',a'}} V^{\pi}(s')  \rvert \\
& \leq \epsilon_{z} + \frac{r_{\max}\gamma}{1-\gamma} \left\| P_{s,a} - P_{s',a'} \right\|_1 \leq \frac{r_{\max}\epsilon_{z}}{1-\gamma},
\end{align*} where we use the assumption that $\phi(s,a) = \phi(s',a') = z$, and the fact that value function $\|V\|_{\infty} \leq r_{\max}/(1-\gamma)$ as $r\sa\in [0, r_{\max}]$.
\end{proof}

Recall the definition $\epsilon_{misspec}(z) = \max_{a} \epsilon_{z}$.

Now we can bound the transfer error defined in \pref{ass:transfer_bias}.
%We leverage the general result in \pref{thm:detailed_bound_rmax_pg} to prove \pref{thm:state_aggregation} by giving a specific bound on $\varepsilon_{bias}$.

\begin{lemma}[Bounding Transfer error] Consider an arbitrary comparator $\pi^\star$ with $d^{\star}(s,a) := d^{\pi^\star}(s) \text{Unif}_{\Acal}(a)$.
Throughout \alg, consider any episode $n$, we have:
\begin{align*}
\EE_{\sa \sim d^\star}\left( Q^n(s,a; r+b^n) - \theta^n_\star\sa  \right)^2 \leq \frac{\EE_{\sa\sim d^\star} [\epsilon^2_{misspec}(\phi\sa)] }{ (1-\gamma)^4},
\end{align*} %where $A^t_\star\sa = \theta^t_\star\cdot \phi\sa - \EE_{a'\sim \pi^t_s} \theta^t_\star\cdot \phi(s,a')$, 
where $\theta^t_\star$ is one of the best on-policy fit:
\begin{align*}
\theta^t_\star \in \arg\min_{\|\theta\|\leq W}\EE_{ \sa\sim \rho^n_{\mix}} \left(\theta\cdot\phi\sa - Q^n(s,a; r+b^n)\right)^2.
\end{align*}\label{lem:bias_in_state_agg}
\end{lemma}
\begin{proof}
Recall that notation $Q^n_{b^n}\sa$ is in short of $Q^n(s,a; r+b^n)$.
First note that as $b^n\sa \in [0,1/(1-\gamma)]$, we must have $Q^n_{b^n}\sa \in [1, 1/(1-\gamma)^2]$.  Second, for any $s,a$ such that $\phi\sa = \phi(s',a') = z$,  we have $\phi(s,a) = \phi(s',a')$ which means that $\sa\in \Kcal^n$ if and only if $(s',a')\in\Kcal^n$ as their features are identical.  This means that the reward misspecification assumption still holds under model $\mathcal{M}_{b^n}$, i.e., $\lvert r(s,a) + b^n(s,a) - r(s',a') - b^n(s',a') \rvert \leq \epsilon_{z}$.

Now let us consider $\theta^t_{\star}$. Using the definition of the state aggregation, we have:
\begin{align*}
&\EE_{ \sa\sim \rho^n_{\mix}} \left(\theta\cdot\phi\sa - Q^n_{b^n}\sa\right)^2 \\
&= \EE_{\sa\sim \rho^n_{\mix}} \sum_{z} \one\{\phi(s,a) = z\} \left( \theta_{z} - Q^n_{b^n}\sa \right)^2,
%& = \EE_{}
\end{align*} which means that for $\theta^t_{\star}$, we have:
\begin{align*}
\sum_{s,a} \rho^n_{\mix}(s,a) \one\{\phi(s,a) = z\} \left( \theta_{z} - Q^n_{b^n}(s,a)\right) = 0,
\end{align*} which implies that $\theta^t_{\star, z} := \frac{  \sum_{s,a} \rho^n_{\mix}(s,a)\one\{\phi(s,a) = z\}  Q^n_{b^n}(s,a)}{ \sum_{s,a}\rho^n_{\mix}(s,a)\one\{\phi(s,a) = z\} } $.
Hence, for any $s'',a'' $ such that $\phi(s'',a'') = z$, we must have:
\begin{align*}
&\left\lvert \theta_{\star, z} - Q^{n}_{b^n}(s'', a'') \right\rvert \\
& = \left\lvert  \frac{  \sum_{s,a} \rho^n_{\mix}(s,a)\one\{\phi(s,a) = z\}  Q^n_{b^n}(s,a)}{ \sum_{s,a}\rho^n_{\mix}(s,a)\one\{\phi(s,a) = z\} }  - Q^n_{b^n}(s'',a'')  \right\rvert\\
& = \left\lvert  \frac{\sum_{s,a} \rho^n_{\mix}(s,a)\one\{\phi(s,a) = z\} \left( Q^n_{b^n}(s,a) - Q^n_{b^n}(s'',a'') \right)}{ \sum_{s,a}\rho^n_{\mix}(s,a)\one\{\phi(s,a) = z\} }         \right\rvert
%& \leq \left\vert  \frac{  \sum_{s,a'} \rho^n_{\mix}(s,a')\one\{\phi(s) = z, a' = a\}  Q^n_{b^n}(s'',a)}{ \sum_{s,a'}\rho^n_{\mix}(s,a')\one\{\phi(s) = z, a'= a\} }  -  Q^{n}_{b^n}(s'', a)  \right\rvert \\
%& \qquad + \left\lvert   \frac{  \sum_{s,a'} \rho^n_{\mix}(s,a')\one\{\phi(s) = z, a' = a\}  (Q^n_{b^n}(s'',a)  - Q^n_{b^n}(s,a))}{ \sum_{s,a'}\rho^n_{\mix}(s,a')\one\{\phi(s) = z, a'= a\} }     \right\rvert \\
 \leq \frac{\epsilon_{z}}{ (1-\gamma)^2  },
\end{align*} where we use Claim~\ref{claim:state_agg}.

%\alekh{I don't follow the additional $1/(1-\gamma)$ factor here? It seems like you plugin C.10 directly and since the bonus is identical in the $s,a$ and $s'',a$ as you show above, there is no blowup by any factors?}

%\begin{align*}
%\theta^t_{\star, z,a} =  \EE_{s\sim \rho^n_{\mix}} \one\{\phi(s) = z\} Q^t_{b^n}\sa,
%\end{align*}
Note $|\theta^n_{\star,z}| \leq \frac{1}{(1-\gamma)^2}$ and $\|\theta^n_\star\|_2 \leq \sqrt{\frac{Z}{(1-\gamma)^4}} := W$ in this case.%\alekh{There is some $\ell_2$ versus $\ell_\infty$ confusion here?}

Now for any state-action distribution $d$, we will have:
\begin{align}
&\EE_{\sa\sim d} \left(Q^n_{b^n}\sa -\theta^n_\star\cdot \phi\sa \right)^2 \nonumber \\
& = \sum_{z} \EE_{\sa\sim d} \one\{\phi(s,a) = z\} \left( Q^n_{b^n}(s,a) - \theta^n_{\star,z} \right)^2 \nonumber\\
& \leq \EE_{(z)\sim d} \frac{\epsilon_{z}^2}{(1-\gamma)^4} \nonumber \leq \frac{\EE_{z\sim d} \epsilon_{misspec}(z)^2 }{(1-\gamma)^4} = \frac{\EE_{\sa\sim d}\left[ \epsilon_{misspec}(\phi(s,a))^2\right] }{(1-\gamma)^4}.
%& \leq \sum_{z} \EE_{\sa\sim d} \one\{\phi(s) = z\} \left\lvert Q^t_{b^n}(s,a) - \theta^n_{\star,z,a} \right\rvert \nonumber \\
%& \leq \sum_{z} \EE_{\sa\sim d} \one\{\phi(s) = z\} \one\{s\in\Kcal^n\} \frac{\epsilon_{z,a}}{(1-\gamma)^2}  \leq \frac{\EE_{(z,a)\sim d} \left[\epsilon_{z,a}\right]  }{(1-\gamma)^2} \leq \frac{\EE_{z\sim d} [\epsilon_{bias}(z)] }{ (1-\gamma)^2 } \label{eq:d_err_state_agg}
\end{align} %where $\epsilon_{misspec}(z) = \max_{a} \epsilon_{z,a}$.



%Now for advantage functions, we have:
%\begin{align*}
%&\EE_{\sa\sim d^\star}\one\{s\in\Kcal^n\}\left( A^t_{b^n}\sa - A^t_\star\sa  \right) \\
%& = \EE_{\sa\sim d^\star}\one\{s\in\Kcal^n\}\left( Q^t_{b^n}\sa -\theta^t_\star\cdot \phi\sa \right) +  \EE_{s\sim d^\star, a\sim \pi^t_s} \left( Q^t_{b^n}\sa - \theta^t_\star\cdot \phi\sa \right).
%\end{align*}  Using inequality~\ref{eq:d_err_state_agg} for both terms, we conclude the proof.
\end{proof}


The above lemma (\pref{lem:bias_in_state_agg}) essentially proves that transfer error $\epsilon_{bias} = \frac{\EE_{z\sim d^\star} [\epsilon_{misspec}^2(z)] }{ (1-\gamma)^4 }$.

Now call \pref{thm:detailed_bound_rmax_pg_new} with $\epsilon_{bias} = \frac{\EE_{z\sim d^\star_{}} [\epsilon^2_{misspec}(z)] }{ (1-\gamma)^4 }$, we conclude the proof of \pref{thm:state_aggregation}. 
\qed


\iffalse
\subsection{Application to Mis-specified Linear MDPs}
We consider model mis-specification in linear MDPs, which is defined formally as follows.
\begin{align*}
P(s' | s,a) = \mu(s') \phi\sa + \epsilon_{s,a}, \quad r(s,a) = \theta\cdot\phi\sa + \epsilon_{s,a},
\end{align*} for some $\epsilon_{s,a}\in [0,1]$ for all $\sa$.

The following claim shows that the resulting $Q^{\pi}$ for any policy $\pi$ is approximately linear. 
\begin{claim}Consider any policy $\pi$, and any reward function $r\sa\in [0, r_{\max}]$. For $Q^{\pi}(\cdot,\cdot; r)$, there exists $\theta^\pi$ such that:
\begin{align*}
\left\lvert Q^\pi(s,a; r) - \theta^\pi \cdot \phi\sa  \right\rvert \leq  \quad \forall \sa.
\end{align*}
\end{claim}
\begin{proof}
to do..
\end{proof}

Consider episode $n$ and the augmented feature $\widetilde\phi\sa = [\phi\sa^{\top}, \one\{\sa\not\in\Kcal^n\}]^{\top}$. 
\fi







==> framework.tex <==
%



\section{Framework}
\label{sec:framework}


%
%


A high-level description of our method is given in Algorithm \ref{alg:rmaxpg_general}. The algorithm operates over epochs and grows a set of policies, called the \textit{policy cover}, whose weighted mixture induces a distribution $\rho_\mathrm{cov}$ over states with increasingly wide coverage.
At each epoch $n$, a new policy $\pi_{n+1}$ is optimized using a
reward bonus ${b}^n$ which assigns high reward to states with low coverage
under $\rho_\mathrm{cov}$. Crucially, the algorithm uses
$\rho_\mathrm{cov}$ as a starting distribution to train
$\pi_{n+1}$. This is done by randomly sampling a policy from the
cover, following it for a certain number of steps, and then switching to the policy
being optimized. By initializing the current policy roughly uniformly
over the region of the state space explored so far, the policy is
assured to receive useful gradients for either exploring new parts of
the state space, or optimizing the environment reward.
Once the new policy is trained, it is added to the policy cover and the next epoch begins.


\iffalse
\begin{algorithm}[t]
\begin{algorithmic}[1]
\STATE \textbf{Require}: parameters
\STATE Initialize policy $\pi^{1}$
\FOR{episode $n = 1, \dots $}
        \STATE Design policy weights $\alpha_1,...,\alpha_{n}$
      	\STATE Define $\rho_{\mix}^n = \sum_{i=1}^n \alpha_i d^{\pi_i}_{\mathcal{M}}$ \label{line:mixture}
	\STATE Design exploration reward $\mathbf{b}_n\sa$ for all $\sa$
        \STATE $\pi_{n+1} = \argmin_\pi \mathbb{E}_{s \sim \rho_\mathrm{mix}^n}[V^{\pi, r}(s) + V^{\pi, \mathbf{b}_n}(s)]$
\ENDFOR
\end{algorithmic}
\caption{Rmax-PG}
\label{alg:rmaxpg_general}
\end{algorithm}
\fi

\begin{algorithm}[t]
\begin{algorithmic}[1]
\STATE \textbf{Require}: MDP $\mathcal{M}$
\STATE Initialize policy $\pi^{1}$
\FOR{episode $n = 1, \dots $}
        \STATE Design policy weights $\alpha_1,...,\alpha_{n}$
      	\STATE Define $\rho_{\textrm{cov}}^n = \sum_{i=1}^n \alpha_i d^{\pi_i}$ \label{line:mixture}
	\STATE Design exploration bonus ${b}^n\sa$ for all $\sa$
        \STATE $\pi^{n+1} = \textrm{PolicyOptimizer}(\rho_{\mathrm{cov}}^n,{b}^n)$
     %
\ENDFOR
\end{algorithmic}
\caption{Rmax-PG}
\label{alg:rmaxpg_general}
\end{algorithm}


A simple strategy for constructing $\rho_\mathrm{cov}$ from the policy cover is to weight all policies equally, i.e. setting $\alpha_i=1/n$.
For linear MDPs, we also consider a rebalancing scheme where the policies are weighted to maximize the log-determinant of their mixture distribution's covariance matrix. This ensures that the weighted policy mixture induces as uniform a coverage as possible over the state space.
%
%
%
Policies with small weights can then be
removed from the cover; in our experiments, we found that our
reweighting scheme allocated high weights to a small number of
policies which were sufficient to obtain good coverage.

%


%

%
%
%
%
%
%


\iffalse
In this section, we introduce the general version of our Rmax-PG algorithm, which can be instantiated in different ways (see~\pref{alg:rmaxpg_general}).
At a high level, the algorithm operates over epochs and grows a set of policies which together induce a distribution over states with increasingly large support.
Specifically, the Rmax-PG framework in~\pref{alg:rmaxpg_general} relies on two oracles: a reward bonus oracle and a policy optimization oracle. The key step in Rmax-PG is to maintain the mixture of all previously learned policies $\rho_{\textrm{cov}}^n$ (\pref{line:mixture}) and call policy optimization (e.g., Natural Policy Gradient) with $\rho_{\textrm{cov}}^n$ as the restart distribution.  Maintaining a mixture of all previously learned policies and always restarting with $\rho_{\textrm{cov}}^n$ to optimize new policy alleviate the forgetting issue: the policy mixture always remembers the previously explored the state-action space. The reward bonus $\mathbf{b}\sa$ is often related to whether or not $\sa$ has been visited many times. Adding sufficient reward bonus (hence name Rmax) encourages the agent to explore to new state action space which may not be covered by the current policy mixture. With bonus, the policy optimization oracle will not experience vanishing gradient issue caused from potential sparse reward structure in the original MDP.
\fi

Both the reward bonus and the policy optimization procedures can be instantiated in different ways depending on the setting at hand.
The reward bonus should be designed to give high reward to states which are not often visited by the policy cover, and low reward to states with high visitation.
In the tabular setting, inverse counts can be used; in the next section, we discuss reward bonuses for the linear and kernelized settings in detail.
In the general setting, possible choices from the deep learning literature include pseudocounts \citep{bellemare2016pseudocounts}, log-densities under a neural model \citep{ostrovski17count}, prediction errors of a dynamics model \citep{pathak2017curiosity}, or random network distillation \citep{burda2018exploration}, all of which can be fit using data collected by rollouts from policies in the cover. The policy optimization procedure can be instantiated using any policy gradient method, for example A2C or PPO \citep{mnih2016asynchronous, schulman2017proximal}.

%



==> macros.tex <==
\newcommand{\Scal}{\mathcal{S}}
\newcommand{\Acal}{\mathcal{A}}

\newcommand{\vr}{\mathbf{r}}
\newcommand{\eps}{\epsilon}
\newcommand{\book}{book\xspace}
\newcommand{\cX}{\ensuremath{\mathcal{X}}}
\newcommand{\cA}{\ensuremath{\mathcal{A}}}
\newcommand{\cP}{\ensuremath{\mathcal{P}}}
\newcommand{\cR}{\ensuremath{\mathcal{R}}}
\newcommand{\Xset}{\ensuremath{\mathcal{X}}}
\newcommand{\Aset}{\ensuremath{\mathcal{A}}}
\newcommand{\dist}{\ensuremath{D}}
\newcommand{\R}{\ensuremath{\mathbb{R}}}
%
%
%
\newcommand{\EE}{\ensuremath{\mathbb{E}}}
\newcommand{\E}{\ensuremath{\mathbb{E}}}
\newcommand{\Eh}{\widehat{\mathbb{E}}}

\renewcommand{\P}{\mathbb{P}}
\newcommand{\F}{\ensuremath{\mathcal{F}}}
\renewcommand{\H}{\ensuremath{\mathcal{H}}}
%
\DeclareMathOperator{\Var}{Var}
%
\DeclareMathOperator{\argmax}{argmax}
\DeclareMathOperator{\argmin}{{argmin}}
\newcommand{\order}{\ensuremath{\mathcal{O}}}
\newcommand{\otil}{\ensuremath{\widetilde{\order}}}
\newcommand{\term}{\ensuremath{\mathcal{T}}}
\DeclareMathOperator{\BiasBdOp}{Bias}
\newcommand{\BiasBd}{\widehat{\BiasBdOp}}

\newcommand{\matM}{\mathbf{M}}
\newcommand{\vf}{\mathbf{f}}
\newcommand{\tvr}{\mathbf{\tilde{r}}}
\newcommand{\tr}{\tilde{r}}

\newcommand{\regret}{\ensuremath{\mathrm{Regret}}}
\newcommand{\reg}{\ensuremath{\mathrm{Reg}}}
\newcommand{\regh}{\ensuremath{\mathrm{\widehat{Reg}}}}
\newcommand{\vb}{\ensuremath{\mathbf{b}}}
\newcommand{\minprob}{\ensuremath{\gamma}}

\newcommand{\greedy}{\textsc{Greedy}\xspace}
\newcommand{\hedge}{\textsc{Hedge}\xspace}
\newcommand{\hedgep}{\ensuremath{\mathbf{p}}}
\newcommand{\hedgew}{\ensuremath{\mathbf{w}}}
\newcommand{\hedgeu}{\ensuremath{\mathbf{u}}}
%

\newcommand{\pihat}{\ensuremath{\widehat{\pi}}}
\newcommand{\w}{w}
\newcommand{\wmax}{\w_{\max}}
\newcommand{\hw}{\hat{w}}%
\newcommand{\hwmax}{\hw_{\max}}
\newcommand{\hr}{\hat{r}}%
\newcommand{\sr}{r^*}
\newcommand{\rmax}{R_{\max}}
\newcommand{\hV}{\hat{V}}%
\newcommand{\Xbar}{\ensuremath{\overline{X}}}
\newcommand{\event}{\ensuremath{\mathcal{E}}}
\newcommand{\piopt}{\ensuremath{\pi^\star}}
\newcommand{\ind}{\ensuremath{\mathds{1}}}
\newcommand{\alg}{\ensuremath{\operatorname{\mathtt{A}}}}

\newcommand{\Rexp}{\ensuremath{v}}%
\newcommand{\Rest}{\ensuremath{\widehat{v}}}%
\newcommand{\Rpred}{\ensuremath{\widetilde{v}}}%
\newcommand{\ips}{\ensuremath{\texttt{\upshape IPS}}\xspace}
\newcommand{\dm}{\ensuremath{\texttt{\upshape DM}}\xspace}
\newcommand{\dr}{\ensuremath{\texttt{\upshape DR}}\xspace}
\newcommand{\switch}{\ensuremath{\texttt{\upshape SWITCH}}\xspace}
\newcommand{\Vhat}{\ensuremath{\widehat{V}}}
\newcommand{\mse}{\textup{\mdseries MSE}}

\newcommand{\AMO}{\ensuremath{\mathcal{AMO}\xspace}}
\newcommand{\pe}{\textsc{PolicyElimination}\xspace}


\newcommand{\pigood}{\ensuremath{\pi_{\textrm{good}}}}
\newcommand{\pibad}{\ensuremath{\pi_{\textrm{bad}}}}

\newcommand{\op}{\ensuremath{\mathsf{OP}}\xspace}
\newcommand\iltcb{\ensuremath{\mathsf{I LOVE TO CON BANDITS}}\xspace}

\newcommand{\Sset}{\ensuremath{\mathcal{S}}}
\newcommand{\Trans}{\ensuremath{P}}
\newcommand{\Rdist}{\ensuremath{r}}
\newcommand{\init}{\ensuremath{\nu}}
\newcommand{\Vstar}{\ensuremath{V^\star}}
\newcommand{\Qstar}{\ensuremath{Q^\star}}

\newcommand{\rmaxalg}{\textsc{R-Max}\xspace}
\newcommand{\rmaxe}{\textsc{R-Max-E}\xspace}
\newcommand{\rmaxg}{\textsc{R-Max-$\gamma$}\xspace}
\newcommand{\inith}{\ensuremath{\widehat{\init}}}
\newcommand{\Transh}{\ensuremath{\widehat{\Trans}}}
\newcommand{\Rdisth}{\ensuremath{\widehat{\Rdist}}}
\newcommand{\Mhat}{\ensuremath{\widehat{M}}}

\newcommand{\rhat}{\ensuremath{\widehat{r}}}

%
\theoremstyle{theorem}
\newtheorem{theorem}{Theorem}[section]
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{claim}[theorem]{Claim}
\theoremstyle{definition}
\newtheorem{assumption}[theorem]{Assumption}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{example}[theorem]{Example}
\newtheorem{remark}[theorem]{Remark}
\newtheorem*{lemma*}{Lemma}
%
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{fact}[theorem]{Fact}
\renewenvironment{proof}{{\bf Proof:}}{\hfill\rule{2mm}{2mm}}
\newcommand{\Assume}[1]{Assumption~\ref{assume:#1}}
\newcommand{\Cor}[1]{Corollary~\ref{cor:#1}}
\newcommand{\Fig}[1]{Figure~\ref{fig:#1}}
\newcommand{\Eq}[1]{Equation~\ref{eq:#1}}
\newcommand{\Sec}[1]{Section~\ref{sec:#1}}
\newcommand{\Thm}[1]{Theorem~\ref{thm:#1}}

%
\newcommand{\card}[1]{\lvert#1\rvert}
\newcommand{\set}[1]{\{#1\}}
\newcommand{\Set}[1]{\left\{#1\right\}}
\newcommand{\bigSet}[1]{\bigl\{#1\bigr\}}
\newcommand{\BigSet}[1]{\Bigl\{#1\Bigr\}}
\newcommand{\braces}[1]{\{#1\}}
\newcommand{\Braces}[1]{\left\{#1\right\}}
\newcommand{\bigBraces}[1]{\bigl\{#1\bigr\}}
\newcommand{\BigBraces}[1]{\Bigl\{#1\Bigr\}}
\newcommand{\bracks}[1]{[#1]}
\newcommand{\bigBracks}[1]{\bigl[#1\bigr]}
\newcommand{\BigBracks}[1]{\Bigl[#1\Bigr]}
\newcommand{\biggBracks}[1]{\biggl[#1\biggr]}
\newcommand{\BiggBracks}[1]{\Biggl[#1\Biggr]}
\newcommand{\Bracks}[1]{\left[#1\right]}
\newcommand{\parens}[1]{(#1)}
\newcommand{\Parens}[1]{\left(#1\right)}
\newcommand{\bigParens}[1]{\bigl(#1\bigr)}
\newcommand{\BigParens}[1]{\Bigl(#1\Bigr)}
\newcommand{\biggParens}[1]{\biggl(#1\biggr)}
\newcommand{\BiggParens}[1]{\Biggl(#1\Biggr)}
%
\newcommand{\given}{|}
\newcommand{\bigGiven}{\mathbin{\bigm\vert}}
\newcommand{\BigGiven}{\mathbin{\Bigm\vert}}
\newcommand{\biggGiven}{\mathbin{\biggm\vert}}
\newcommand{\Norm}[1]{\left\lVert#1\right\rVert}
\newcommand{\bigNorm}[1]{\bigl\lVert#1\bigr\rVert}
\newcommand{\BigNorm}[1]{\Bigl\lVert#1\Bigr\rVert}
\newcommand{\norm}[1]{\lVert#1\rVert}
\newcommand{\abs}[1]{\lvert#1\rvert}
\newcommand{\Abs}[1]{\left\lvert#1\right\rvert}
\newcommand{\bigAbs}[1]{\bigl\lvert#1\bigr\rvert}
\newcommand{\BigAbs}[1]{\Bigl\lvert#1\Bigr\rvert}
\newcommand{\biggAbs}[1]{\biggl\lvert#1\biggr\rvert}
\newcommand{\angles}[1]{\langle#1\rangle}
\newcommand{\floors}[1]{\lfloor#1\rfloor}
\newcommand{\Floors}[1]{\left\lfloor#1\right\rfloor}
\newcommand{\ceils}[1]{\lceil#1\rceil}
\newcommand{\Eu}[1]{\underset{#1}{\E}}

\newcommand{\Vcal}{\ensuremath{\mathcal{V}}}
\newcommand{\Vcalh}{\ensuremath{\widehat{\mathcal{V}}}}
\newcommand{\Qtil}{\ensuremath{\tilde{Q}}}
\newcommand{\zhat}{\ensuremath{\hat{z}}}
\newcommand{\Vghat}{\ensuremath{{\Vhat}^\gamma}}
\newcommand{\err}{\ensuremath{\text{err}}}
\newcommand{\Hcal}{\ensuremath{\mathcal{H}}}
\newcommand{\Bell}{\ensuremath{\mathcal{T}}}
\newcommand{\Phat}{\ensuremath{\widehat P}}
\newcommand{\Bellh}{\ensuremath{\widehat \Bell}}
\newcommand{\calF}{\ensuremath{\mathcal{F}}}
\newcommand{\loss}{\ensuremath{\mathcal{L}}}
\newcommand{\lossh}{\ensuremath{\widehat{\loss}}}
\newcommand{\Qh}{\ensuremath{\widehat{Q}}}
\newcommand{\pitil}{\ensuremath{\widetilde{\pi}}}
\newcommand{\bp}{\ensuremath{\theta}}
\newcommand{\cntidx}{\ensuremath{\alpha}}
\newcommand{\bcnt}{\ensuremath{\bm{\cntidx}}}
\newcommand{\idx}{\ensuremath{\beta}}
\newcommand{\bidx}{\ensuremath{\bm{\idx}}}
\newcommand{\hist}{\ensuremath{\text{hist}}}
\newcommand{\mbound}{\ensuremath{\alpha}}
\newcommand{\pmax}{\ensuremath{\bar{p}}}
\newcommand{\pmin}{\ensuremath{\underline{p}}}
\renewcommand{\S}{\ensuremath{\mathbb{S}}}
\newcommand{\kl}{\ensuremath{\mathrm{KL}}}

\DeclareMathOperator{\chd}{child}

\newcommand{\epsopt}{\ensuremath{\eps_{\text{opt}}}}
\newcommand{\epsapp}{\ensuremath{\eps_{\text{approx}}}}
\newcommand{\lbpe}{\ensuremath{L_{\textrm{BPE}}}}
\newcommand{\tepsapp}{\ensuremath{\widetilde\eps_{\textrm{approx}}}}
\newcommand{\Ah}{\ensuremath{\widehat A}}
\newcommand{\wh}{\ensuremath{\widehat w}}
\newcommand{\epsh}{\ensuremath{\widehat{\eps}}}
\newcommand{\diag}{\textrm{diag}}
\newcommand{\ones}{\mathbf{1}}
\newcommand{\iden}{\textrm{I}}
\newcommand{\onesm}{\mathbf{J}}
\newcommand{\Ncal}{\mathcal{N}}
\newcommand{\bigO}{{O}}
\newcommand{\sa}{(s,a)}
\newcommand{\uniform}{\text{Uniform}}
\newcommand{\cgeq}{\succcurlyeq}
\newcommand{\proj}{\mathbf{P}}
\newcommand{\Kbar}{\ensuremath{\overline{K}}}
\newcommand{\bonus}{\omega}
\newcommand{\actidx}{\alpha}
\newcommand{\phitil}{\widetilde{\phi}}
\newcommand{\piterm}{\ensuremath{\pi_+}} 
\newcommand{\tauterm}{\ensuremath{\tau_+}}
\newcommand{\Mcal}{\mathcal{M}}
\newcommand{\trace}{\textsc{Trace}}
\newcommand{\intdim}{\textsc{IntDim}}
\newcommand{\boldpi}{\boldsymbol{\pi}}



==> main_pseudocode.tex <==
\begin{algorithm}[!t]
\begin{algorithmic}[1]
\State \hspace*{-0.1cm}\textbf{Input}: iterations $K$, threshold $\beta$, regularizer $\lambda$, optimization rounds $T$, stepsize $\eta$, sample size $M$
\State \hspace*{-0.1cm}Initialize $\pi^0(a|s)$ to be uniform and estimate its feature covariance matrix $ \widehat\Sigma^0$
\For{episode $n = 0, \dots K-1$}
\State Set $\rho^n_{\mix} = \sum_{i=0}^n d^{\pi^i} / (n+1)$ \label{line:mixture}
\State Obtain $N$ i.i.d. $(s_i, a_i)$ samples from $d^{\pi^n}$ by invoking \Call{$d^\pi$-sampler}{$\pi^n$}. Estimate covariance:
\Statex \hskip\algorithmicindent$\widehat{\Sigma}^n = \sum_{i=1}^N \phi(s_i,a_i)\phi(s_i,a_i)^{\top}/N$ \label{line:feature_cov}
%$\end{center}

\State Estimate covariance of the policy cover as \label{line:feature_cov_mix}
%\begin{center}
 $\widehat\Sigma_\mix \gets \widehat \Sigma_\mix + \widehat{\Sigma}^n =  \sum_{i=0}^n  \widehat\Sigma^i + \lambda \mathbf{I}$ \label{eq:covariance_est}
%\end{center}
\vspace*{0.1cm}
	\State Set the exploration bonus $b^n$~\eqref{eq:bonus} to reward infrequently visited directions under $\rho^n_{\mix}$\label{line:bonus}
\For{iteration $t = 0, \dots T-1 $}\label{line:for_beg}
    \State \parbox[t]{350pt}{Draw $M$ i.i.d. samples by drawing $i\in[N]$ u.a.r, executing $\pi_i$ for $h$ steps with probability $\gamma^h$ to get $(s_i, a_i)$ and then continuing with $\pi$ for $h_1$ more steps with probability $\gamma^{h_1}$. Set $\hat{Q}^t(s_i, a_i;b^n)$ as the undiscounted return in the later $h_1$ steps\strut}
	\State \textbf{Critic}: \label{line:learn_critic}\vspace*{-0.5cm}
	\begin{align*}
		\theta^t = \argmin_{\|\theta\|\leq W} \sum_{i=1}^M ( \theta\cdot  \phi(s_i,a_i) - \widehat{Q}^{t}(s_i,a_i;b^n) )^2%,\\
	\end{align*}
\Statex \hskip \algorithmicindent \hskip \algorithmicindent where $s_i,a_i\sim \rho$, and $\widehat{Q}^t (s_i,a_i;b^n)$'s are unbiased estimates of $Q^{t}(s_i,a_i;b^n)$
\vspace*{0.1cm}
	\State \textbf{Actor} update via exponential gradient, for $s$: \label{line:learn_actor}
    %\IF{$s\in \Kcal$}
    %\STATE
	\begin{eqnarray*}
		%\hspace{-0.2in}
\pi^{t+1}(\cdot|s) &\propto& \pi^t(\cdot |s) \exp\left(\eta \theta^t\cdot \phi(s,\cdot)\right),  \quad
\textrm{if } \forall a'\in \Acal,  \,  b^n(s,a') = 0,\\%\end{eqnarray*}
%\vspace*{-0.5cm}
%\begin{eqnarray*}
\pi^{t+1}(\cdot|s) &=& \text{Uniform}\left(\{a: b^n(s,a) \neq 0\}\right), \quad\mbox{otherwise}.\qquad\qquad\qquad\qquad
%\pi^{t+1}(\cdot|s) &=& \text{Uniform}\left(\{a:\sa\not\in\calK\}\right), \quad\mbox{otherwise}.\qquad\qquad\qquad\qquad
	\end{eqnarray*}
%\ENDIF
	%
	%
	\EndFor\label{line:for_end}
\State Set $\pi^{n+1} = \pi^T$
\EndFor
\vspace*{0.2cm}
\Function{$d^\pi$-sampler}{$\pi$}
\State Sample $h\in \mathbb{N}$ with probability $\gamma^h$
\State Execute $\pi$ in the MDP starting from initial state $s_0$
\State \Return $(s_h, a_h)$
\EndFunction
\end{algorithmic}
\caption{\AlgLong (\alg)}
\label{alg:epoc}
\end{algorithm}



==> proof_techniques.tex <==
\subsection{Key Lemmas}
\label{sec:proof_tech}

In this section, we highlight some of key lemmata that we use to analyze \alg. The key technical lemma is the following NPG-like convergence result but with an extra term that relates to the accumulative bonuses collected by \alg.

\begin{lemma}[\alg Convergence]
For an arbitrary comparator policy $\pi^\star$, under \pref{ass:transfer_bias}, and the following condition: for all $n$,
\begin{align*}
\EE_{\sa\sim \rho_{\mix}^n}\left( Q^n(s,a; r+b^n) -  \theta^n\cdot \phi\sa \right)^2 \leq  \min_{\theta:\|\theta\|\leq W} \EE_{\sa\sim \rho_{\mix}^n}\left( Q^n(s,a; r+b^n) -  \theta\cdot \phi\sa \right)^2 + \epsilon_{stat},
\end{align*} where $\epsilon_{stat} \in \mathbb{R}^+$, then we have:
\begin{align*}
V^{\pi^\star}  - \max_{n\in [0,\dots, N-1]} V^n &
 \leq  \frac{1}{1-\gamma}\left(\sqrt{\frac{4W^2\log(A)}{N}} + 2\sqrt{A\epsilon_{bias}} + 2\sqrt{ \beta  \lambda W^2  } + 2\sqrt{\beta N \epsilon_{stat}}\right) \\
&\qquad + \frac{1}{N} \sum_{n=0}^{N-1} \EE_{\sa\sim d^{n}}\left[b^n\sa \right].
\end{align*}
\label{lem:epoch_convergence}
\end{lemma}
Note that $\epsilon_{stat}$ is the generalization error from constrained linear regression which often scales in the order of $O(\text{poly}(W)/\sqrt{M})$ with $M$ being the number of samples used for linear regression. The threshold $\beta$ is set to be $O(\text{poly}(\epsilon))$.

%To prove the above lemma, we need to construct absorbing MDPs based on the so-called known set $\calK^n = \{\sa: b^n\sa > 0\}$.

%While the NPG algorithm has been analyzed in some prior works~\citep{geist2019theory,agarwal2019optimality,shani2019adaptive}, most of these analyses use either an $\ell_\infty$ bound on the density ratio between the initial state distribution of NPG and the comparison policy, or even stronger concentrability coefficients. None of these quantities are small during the execution of \pref{alg:npg} under our assumptions in general. Here, we present a different analysis which builds on that of~\citet{agarwal2019optimality}, and uses a transfer bias resulting from a change in distributions for fitting the critic. Crucially, this transfer error is always bounded.

Comparing to Q-NPG in \cite{agarwal2019optimality}, we note that \alg completely eliminates the need of an initial distribution with a nontrivial condition number (see Remark~\ref{remark:compare_to_Q_npg}). %, i.e., \cite{agarwal2019optimality} assumes that $\kappa := \tr\left( \EE_{\sa\sim d^\star}\phi\sa\phi\sa \left(\EE_{s,a\sim \rho_0} \phi\sa\phi\sa^{\top}\right)^{-1}\right) < \infty$ and their bound explicitly depends on $\kappa$ which could be exponentially large even in tabular setting.
 Instead, \alg's convergence result contains a new term which is the average expected reward bonuses collected by the sequence of learned policies.
%Hence, we present a different analysis which builds on that of~\citet{agarwal2019optimality}, and uses a transfer bias resulting from a change in distributions for fitting the critic. Crucially, this transfer error is always bounded. We also specialize the NPG analysis in linear function approximation setting here so that we can use a condition number type of guarantee rather than distribution mismatch ratio.
%In addition to transfer bias, another difference between the classic convergence result of NPG and \pref{lem:epoch_convergence} is that \pref{lem:epoch_convergence} has a term which is the average expected reward bonus collected across $N$ rounds.
The next lemma shows that the accumulative reward bonus scales in the order of information gain $\mathcal{I}_N(1)$ (e.g., in finite dimensional setting with bounded feature norm, $\mathcal{I}_N(1)$ scales as $O(d\log(N+1))$). %in the order of $d \log( N)$ under the simplified assumption that $\phi\in\mathbb{R}^d$ (it can be extended to infinite dimensional setting using intrinsic dimension $\widetilde{d}$).
\begin{lemma}[Information Gain and Average Reward Bonus]
Consider any sequence of policies $\pi^0, \cdots \pi^{N-1}$ for any $N$, we have:
\begin{align*}
\frac{1}{N }\sum_{n=0}^{N-1} \EE_{\sa\sim d^{n}} \left[ b^n \sa \right] \leq \frac{\mathcal{I}_N(1)}{N \beta (1-\gamma)}.
\end{align*}
\end{lemma}
Hence, for a large $N$ (large enough to offset $\beta(1-\gamma)$ where $\beta = O(\text{poly}(\epsilon))$), the average reward bonus will converge to zero as maximum information gain grows sublinearly for common kernels \citep{srinivas2010gaussian}.

Combining the above two lemmas, we get to the following convergence result of \alg:
\begin{align*}
&V^{\pi^\star}  - \max_{n\in [0,\dots, N-1]} V^n \\
& \leq  \frac{1}{1-\gamma}\left(\sqrt{\frac{4W^2\log(A)}{N}} + 2\sqrt{A\epsilon_{bias}} + 2\sqrt{ \beta  \lambda W^2  } + 2\sqrt{\beta N \epsilon_{stat}}\right)  + \frac{\mathcal{I}_N(1)}{N\beta(1-\gamma)}.
 \end{align*}



The final proof of \pref{thm:agnostic} consists of combining the above two lemmas and setting parameters ($N, \beta, \lambda, \epsilon_{bias}$) properly to be $O(\epsilon + \sqrt{A\epsilon_{stat}}/(1-\gamma))$ close to $\pi^\star$.  %Roughly, this means that we need to set $N \approx 1/(\epsilon(1-\gamma))^2$, $\beta \approx \epsilon^2$,
The detailed proof is included in \pref{app:analysis}.


%Briefly, we can set




==> resubmission.tex <==
This work was submitted to ICML 2020. Since the submission, we have made substantial changes and improvements to the paper. Below we first summarize the ICML reviews and then discuss the changes that we have made.

We had three weak accepts and one weak reject. The weak reject reviewer, in our perspective, got confused about our new exploration algorithm with the existing policy gradient algorithms which do not  explore (e.g., NPG, TRPO). Though we explicitly pointed out that NPG/TRPO are not PAC algorithms even in tabular setting while ours is in the rebuttal, the reviewer did not update their review after the rebuttal. The other three reviewers who gave weak accepts were generally positive, but they thought our method is a straightforward combination of Rmax [R. I. Brafman and M. Tennenholtz, JMLR] and NPG [Agarwal et.al, 19]. They were also curious about how our model misspecification results are comparable to classic concepts such as concentrability coefficients. 

Based on the reviews from ICML, we made the following major improvements in this new version. 

First, we changed our algorithm's name and the paper's title to better reflect three key properties of the our new algorithm (exploration, policy optimization, and policy cover).

Second, we included a specific discussion on model-misspecification due to state-aggregation. We gave an example which has model misspecification due to state aggregation, and we show that our algorithm achieves a local L_{infinity} type of error guarantee while existing value/model-based algorithms suffer L_{infinity} error which is the maximum possible model misspecification over the entire state space. Specifically, we illustrate that our local L_infinity error is the averaged model misspecification under a fixed comparator policy (e.g., the best policy in policy class). We hope this simple example illustrates the potential benefits of our method in the agnostic setting over value-based approaches.

Third, we included a table in the introduction to explicitly compare our approach to existing works, including sample efficient model-based RL algorithms, sample efficient model-free algorithms, and especially existing policy gradient algorithms. Specifically we point out that existing PG algorithms require a good initial distribution in order to guarantee performance, while our algorithm does not and instead explicitly constructs a policy cover to overcome this exploration challenge. We emphasize that in tabular and linear MDP settings, our algorithm finds a near optimal policy in polynomial sample complexity while existing PG methods such as NPG need to satisfy some initial state condition in order to achieve near optimality. 

We also prove a new theorem for reward-free exploration (i.e., reward is zero everywhere and the agent thus aims to explore the entire state space as quickly as possible) and experimentally verify our approach in a reward-free maze environment. Since existing PG methods do not make progress in reward free setting (i.e., gradient is zero), we hope this highlights the difference between our PG method and the existing ones from both theoretical and experimental perspectives. 

Fourth, we updated the related work section. During the review process of ICML, we noticed that a related concurrent paper ``Provably Efficient Exploration in Policy Optimization" Cai et.al, 19 was posted on arXiv. To better position our work, we studied the paper and we added a discussion to compare to this work. While this paper got into ICML, unfortunately we noticed that their proof has a significant bug which makes that the main results do not hold (this was confirmed with the authors of this paper). We thus discussed this paper explicitly in the related work and also pointed out the specific bug in the appendix.

Finally, we also improved writing by explicitly pointing out what objectives our PG algorithm is optimizing, adding the intuition of our reward bonuses when specialized to tabular setting, and explaining the explicit NPG policy parameter update step in the algorithm pseudocode.





==> tmp.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=.6\textwidth]{media/tree_example5}
\caption{The binary tree example. Note that here $s_0$ and $s_1$ have features only span in the first three standard basis, and the features for states inside the binary tree (dashed) contains features in the null space of the first three standard bases. Note that the features inside the binary tree could be arbitrary complicated. Unless the feature dimension scales $\exp(H)$ with $H$ being the depth of the tree, we cannot represent this problem in linear MDPs. The on-policy nature of \alg ensures that it succeeds in this example. Due to the complex features and large $\ell_{\infty}$ model-misspecification inside the binary tree, Bellman-backup based approaches (e.g., Q-learning) cannot guarantee successes.}
\label{fig:binary_tree}
\end{figure}

%\subsection{Robustness to ``Delusional Bias'' with Partially Correct Models}
\subsection{Robustness to ``Delusional Bias'' with Partially Well-specified Models}

%\subsection{Construction}

In this section, we provide an additional example of model
misspecification where we show that \alg succeeds while Bellman backup
based algorithms do not. The basic spirit of the example is that if
our modeling assumption holds for a sub-part of the MDP, then \alg can
compete with the best policy that only visits states in this sub-part
with some additional assumptions. In contrast, prior model-based and
$Q$-learning based approaches heavily rely on the modeling assumptions
being globally correct, and bootstrapping-based methods
%(e.g.~\citep{jin2019provably}) 
fail in particular due to their
susceptibility to the delusional bias problem~\citep{lu2018non}. 

We emphasize that this constructed MDP and class of features have the following properties:

\begin{itemize}
\item It is not a linear MDP; we would need the dimension to be exponential in the depth $H$, i.e. $d=\Omega(2^H)$, in order to even approximate the MDP as a linear MDP.
\item Value based or model based algorithms that rely on Bellman
  backup (e.g., Q learning) will fail, unless they satisfy an agnostic
  approximation condition which no known algorithms are known to have.
\item Our example will have large worst case function approximation
  error, i.e. the $\ell_{\infty}$ error in approximating $Q^\star$
  will be (arbitrarily) large.
\item The example can be easily modified so that the concentrability
  coefficient (and the distribution mismatch coefficient) of the
  starting distribution (or a random initial policy)   will be
  $\Omega(2^H)$.
\end{itemize}

Furthermore, we will see that \alg succeeds on this example, provably. 
%The example
%highlights the improved approximation power of policy gradient methods,
%when used in conjunction with our ``on-policy", policy cover approach.

We describe the construction below (see \pref{fig:binary_tree} for an example). There are two actions, denoted by $L$ and $R$. At initial state $s_0$, we have
$P(s_1 | s_0, L) = 1$; $P(s_1 | s_1, a) = 1$ for any $a\in \{L, R\}$. We set the reward of taking the left action at $s_0$ to be $1/2$, i.e.  $r(s_0,L)=1/2$.
This implies that there exists a policy which is guaranteed to obtain at least reward $1/2$.
When taking action $a= R$ at $s_0$, we deterministically transition
into a depth-H completely balanced binary tree.     We can further
constrain the MDP so that the optimal value is $1/2$ (coming from left
most branch), though, as we see later, this is not needed.

%and optimal policy $\pi^\star(s_0) = L$

The feature construction of $\phi\in \mathbb{R}^d$ is as follows: For
$s_0, L$, we have $\phi(s_0, L) = e_1$ and
$\phi(s_0, R) = e_2$, and $\phi(s_1, a) = e_3$ for any $a\in\{L,R\}$,
where $e_1, e_2, e_3$ are the standard basis vectors. For all other
states $s\not\in\{s_0,s_1\}$, we have that $\phi\sa$ is constrained to be
orthogonal to $e_1$, $e_2$, and $e_3$, but otherwise arbitrary. In
other words, $\phi\sa$ has the first three coordinates equal to zero
for any $s\not\in \{s_0,s_1\}$ but can otherwise be pathological.

The intuition behind this construction is that the features $\phi$
are allowed to be arbitrary complicated for states inside the
depth-H binary tree, but are uncoupled with the features
on the left path. This implies that both \alg and any other algorithm do
not have access to a good global function approximator.

Furthermore, as discussed in the following remark, these features do not provide a good approximation of the true dynamics as a linear MDP.

\begin{remark}(Linear-MDP approximation failure). As the MDP is
  deterministic, we would need dimension $d =
\Omega(2^H)$ in order to approximate the MDP as a linear MDP (in the
sense required in~\cite{jin2019provably}). This is due to that the rank
of the transition matrix is $O(2^H)$.
\end{remark}

However the on-policy nature of \alg ensures that there always exists a best linear predictor that can predict $Q^{\pi}$ well under the optimal trajectory (the left most path) due to the fact that the features on $s_0$ and $s_1$ are decoupled from the features in the rest of the states inside the binary tree. Thus it means that the transfer error is always zero. This is formally stated in the following lemma.
\begin{corollary}[Corollary of Theorem~\ref{thm:agnostic}]
\alg is guaranteed to find a policy with value greater than $1/2-\epsilon$
with probability greater than $1-\delta$, using a number of samples
that is $O\left(\textrm{poly}(H,d, 1/\epsilon,\log(1/\delta))\right)$. This is due to
the transfer error being zero.
\label{cora:agnostic}
\end{corollary}

We provide a proof of the corollary in~\pref{app:examples}. 

\paragraph{Intuition for the success of \alg.} Since the corresponding
features of the binary
subtree have no guarantees in the worst-case, \alg may not successfully find the
best global policy in general. However, it does succeed in finding a
policy competitive with the best policy that remains in the
\emph{favorable} sub-part of the MDP satisfying the modeling
assumptions (e.g., the left most trajectory in
\pref{fig:binary_tree}). We do note that the feature orthogonality is
important (at least for a provably guarantee), otherwise the errors in fitting value functions on the
binary subtree can damage our value estimates on the favorable parts
as well; this behavior effect may be less mild in practice. 

\paragraph{Delusional bias and the failure of Bellman backup-based
  approaches.} As remarked above, no algorithm can hope to reliably
estimate the value functions in the binary subtree accurately with a
polynomial sample complexity, due to that we are not assuming any
guarantees about the quality of the features in that part of the
subtree. Furthermore, there is a no evidence that prior exploration approaches relying on Bellman
backups will not overestimate the values from
this subtree, due to the uncontrolled approximation error.
 Even parametric model based approaches also have
no guarantees if the model parameterization is not accurate in the subtree.
If such an overestimate occurs, then this overestimate will be perfectly
backed up to the root at $s_0, R$,
since we have no loss in expressivity at $s_0, R$ (nor is there interference from
features in any other state-action pairs). Hence, even if the values in
the left path are accurately estimated, the algorithm may incorrectly
favor the right action in the root. 
%Of course it discovers the error
%in its estimation upon executing this policy in the real MDP, but note
%that the trial and error can last for an exponentially large number of
%interactions. 
This example serves to highlight the crucial limitations
of Bellman backups when considering actions that lead to places of
model misspecification, quite like the issues highlighted
in~\citet{lu2018non}. 

\paragraph{Failure of concentrability-based approaches} Some of the
prior results on policy optimization algorithms, starting from the
Conservative Policy Iteration
algorithm~\citet{kakade2002approximately} and further studied in a
series of subsequent
papers~\citep{Scherrer:API,geist2019theory,agarwal2019optimality}
provide the strongest guarantees in settings without exploration, but
considering function approximation. As remarked in
Section~\ref{sec:linear}, most works in this literature make
assumptions on the maximal density ratio between the initial state
distribution and comparator policy to be bounded. In the MDP
of~\pref{fig:binary_tree}, this quantity seems fine since the ratio is
at most $H$ for the comparator policy that goes on the left path (by
acting randomly in the initial state). However, we can easily change
the left path into a fully balanced binary tree as well, with $O(H)$
additional features that let us realize the values on the leftmost
path (where the comparator goes) exactly, while keeping all the other
features orthogonal to these. It is unclear how to design an initial
distribution to have a good concentrability coefficient, but \alg
still competes with the comparator following the leftmost path since
it can realize the value functions on that path exactly and the
remaining parts of the MDP do not interfere with this estimation.  

\input{proof_techniques}








==> transfer_bias.tex <==
\subsection{Agnostic Result with Transfer Bias}

To measure the sample complexity, we define the \emph{intrinsic dimension} of the underlying MDP $\mathcal{M}$.
First, denote the covariance matrix of any policy $\pi$ as $\Sigma^{\pi} = \EE_{\sa\sim d^{\pi}}\left[\phi\sa\phi\sa^{\top}\right]$.%
We define the intrinsic dimension below:
\begin{definition}[Intrinsic Dimension $\widetilde{d}$] We define intrinsic dimension as:
%Intrinsic dimension $\widetilde{d}$:
\begin{align*}
\widetilde{d}: =\max_{n\in\mathbb{N}^+} \max_{\{\pi^i\}_{i=1}^n } \frac{  \log\det\left(\sum_{i=1}^n \Sigma^{\pi^i} + \mathbf{I}\right) }{\log(n + 1)}.
\end{align*}
\label{def:int_dim}
\end{definition}
This quantity is identical to the intrinsic dimension in Gaussian
Processes bandits  \citep{srinivas2010gaussian}; one viewpoint of this
quantity is as the information gain from a Bayesian perspective
(\cite{srinivas2010gaussian}). A related quantity occurs in a more
restricted linear MDP model, in \citet{yang2019reinforcement}. Note
that when $\phi\sa\in \mathbb{R}^d$, we have that
$\log\det\left(\sum_{i=1}^n \Sigma^{\pi^i} + \mathbf{I}\right) \leq d
\log(n + 1)$ (as $\|\phi(s,a)\|_2\leq 1$), which means that the
intrinsic dimension is $d$.  Note that $\widetilde{d}\ll d$ if the
covariance matrices from a sequence of policies only concentrated in a
low-dimensional subspace.

%We consider general MDPs where the model mis-specification is modelled in a new concept \emph{transfer bias}. The transfer bias  generalizes the previous two results we discussed above: in linear MDPs, transfer bias is zero, and in state-aggregation, the transfer bias is at most the model-misspecification averaged over the comparator's abstracted state distribution. We define transfer bias as follows:
We introduce transfer bias in the following assumption. 
\begin{assum}[Transfer Bias] \label{ass:transfer_bias} Consider the best comparator policy $\pi^\star\in \Pi_\mathrm{linear}$.
Assume that at any iteration $t$ within any episode $n$, there exits a best on-policy fit:
\begin{align*}
\theta^t_\star \in \argmin_{\|\theta\|\leq W}\EE_{\sa\sim \rho^n_{\mix}} \left( \theta\cdot \phi\sa - Q^t(s,a; r+b^n) \right)^2,
\end{align*} such that its associated critic ${A}^t_\star\sa := \theta^t_\star\cdot \phi\sa - \EE_{a'\sim \pi^t_s} \theta^t_\star\cdot \phi(s,a')$ has a bounded prediction error when transferred to $d^\star_{linear}$:
\begin{align*}
\EE_{\sa\sim d^\star_{linear}}\one\{s\in\Kcal^n\} \left( A^t(s,a; r+b^n) - A^t_\star\sa \right) \leq \varepsilon_{bias} \in \mathbb{R}^+.
\end{align*}
\end{assum}
\begin{remark}[Transfer bias VS Concentrability Coefficient \citep{kakade2002approximately,agarwal2019optimality}]
Note that transfer bias is always finite and in worst case can be upper bounded by concentrability coefficient:
\begin{align*}
\varepsilon_{bias} \leq \sqrt{\left\|\frac{ d^\star_{linear}  }{ \rho^n_{\mix} }\right\|_{\infty} \EE_{\sa\sim \rho^n_{\mix}} \left(A^t(s,a; r+b^n) - A^t_\star\sa \right)^2 },
\end{align*}  assuming the concentrability coefficient $ \left\|{ d^\star_{linear}  }/{ \rho^n_{\mix} }\right\|_{\infty}$ is finite.  The transfer bias is different from concentrability coefficient in a sense that it measures model-misspecification (approximation error of advantage functions) averaged over a fixed comparator distribution $d^\star_{linear}$ rather than in the $\ell_{\infty}$ form which could easily be infinite. 
\end{remark}

With the above assumption on the transfer bias, the next theorem states an agnostic result of \alg:
\begin{theorem}[Agnostic Guarantee of \alg]
Assume \pref{ass:transfer_bias} holds. Fix $\epsilon, \delta \in (0,1)$. Suppose that $\mathcal{M}$ is a linear MDP. %Then $\varepsilon_{bias} = 0$.
There exists a setting of the parameters such that \alg
uses a number of samples at most $\text{poly}\left( \frac{1}{1-\gamma},\log(A), \frac{1}{\epsilon}, \widetilde{d}, W, \ln\left(\frac{1}{\delta}\right) \right)$
and, with probability greater than $1-\delta$, returns a policy $\widehat \pi$ such that:
$V^{\widehat\pi}(s_0) \geq \max_{\pi\in\Pi_\mathrm{linear}}V^{\pi}(s_0) - \epsilon - \frac{\varepsilon_{bias}}{1-\gamma}$. %where $V^{\star}(s_0)$ is the optimal value function.
\label{thm:agnostic}
\end{theorem}

The detailed bound with the rates, along with the setup of
hyperparameters $\beta, \lambda$, $T$, $M$, $\eta$ (learning rate in
NPG) are in~\pref{app:rmaxpg_sample}. Our theorem assumes discrete
actions but the sample complexity only scales polylogarithmically with
respect to the number of actions $A$, making the algorithm scalable to
large action spaces.


The result above shows that we achieve $\epsilon$ near optimal policy if transfer bias is small. Below we show two examples where transfer bias is small (zero in linear MDPs as all Q functions are linear there, and small in state-aggregation).




